The Actor-Critic Update Order Matters for PPO in Federated Reinforcement Learning

In the context of Federated Reinforcement Learning (FRL), applying Proximal Policy Optimization (PPO) faces challenges related to the update order of its actor and critic due to the aggregation step occurring between successive iterations. In particular, when local actors are updated based on local critic estimations, the algorithm becomes vulnerable to data heterogeneity. As a result, the conventional update order in PPO (critic first, then actor) may cause heterogeneous gradient directions among clients, hindering convergence to a globally optimal policy. To address this issue, we propose FedRAC, which reverses the update order (actor first, then critic) to eliminate the divergence of critics from different clients. Theoretical analysis shows that the convergence bound of FedRAC is immune to data heterogeneity under mild conditions, i.e., bounded level of heterogeneity and accurate policy evaluation. Empirical results indicate that the proposed algorithm obtains higher cumulative rewards and converges more rapidly in five experiments, including three classical RL environments and a highly heterogeneous autonomous driving scenario using the SUMO traffic simulator.

==> draft.tex <==
\section{Proof of Lemma \ref{lemma:omega}\label{proof:lemma:omega}}

\begin{proof}
\begin{lemma}
For energy-based policy,
\begin{alignat}{1}
-\Omega_{CA} &= -\sum_{s} \sum_{n} q_{n} \rho_{\pi^{\ast},n}(s) \left< \log \left( \pi^{\theta^{t+1}}(\cdot \vert s) / \pi^{\theta^{t+1}_{n}}(\cdot \vert s) \right), \pi^{\ast} \right> \\
&= \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \log \pi^{\theta_{n}^{t+1}}(s,a) - \log \pi^{\theta^{t+1}}(s,a) \right] \\
&= \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \tau^{-1}_{t+1} f_{\theta_{n}^{t+1}}(s,a) - \tau^{-1}_{t+1} f_{\theta^{t+1}}(s,a) \right] \\
&\le \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \tau_{t+1}^{-1} f_{\theta_{n}^{t+1}}(s,a) - \tau_{t+1}^{-1} f_{\theta^{t+1}}(s,a) \right\vert \right] \\
&\le 2 \mathbb{E}_{n \thicksim C} \left[ \tau_{t+1}^{-1} \epsilon^{t+1}_{n} \xi^{t+1}_{n} \right] + \beta_{t}^{-1} \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \sum_{i} q_{i} \left\vert Q^{w^{t}_{n}}(s,a) - Q^{w^{t}_{i}}(s,a) \right\vert \right] + 2 \mathcal{O} \left( \tau_{t+1}^{-1} R_{\theta}^{3/2} m^{-1/4} \right).
\end{alignat}
For stochastic Gaussian policy,
\begin{alignat}{1}
-\Omega_{CA} &= -\sum_{s} \sum_{n} q_{n} \rho_{\pi^{\ast},n}(s) \left< \log \left( \pi^{\theta^{t+1}}(\cdot \vert s) / \pi^{\theta^{t+1}_{n}}(\cdot \vert s) \right), \pi^{\ast} \right> \\
&= \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \log \pi^{\theta_{n}^{t+1}} - \log \pi^{\theta^{t+1}} \right] \\
&= \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ - \frac{\left( a - f_{\theta^{t+1}_{n}}(s,a) \right)^2}{2 \sigma_{t+1}^{2}} - \log \sqrt{2 \pi} \sigma_{t+1} + \frac{\left( a - f_{\theta^{t+1}}(s,a) \right)^2}{2 \sigma_{t+1}^{2}} + \log \sqrt{2 \pi} \sigma_{t+1} \right] \\
&= \frac{1}{2 \sigma_{t+1}^{2}} \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left( a - f_{\theta^{t+1}}(s,a) \right)^2 - \left( a - f_{\theta^{t+1}_{n}}(s,a) \right)^2 \right] \\
&= \frac{1}{2 \sigma_{t+1}^{2}} \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left( a - f_{\theta^{0}}(s,a) \right)^2 + 2 \left( f_{\theta^{0}}(s,a) - a \right) \left( f_{\theta^{t+1}}(s,a) - f_{\theta^{0}}(s,a) \right) \right. \\
& \quad + 2 \left( f_{\theta^{t+1}}(s,a) - f_{\theta^{0}}(s,a) \right)^{2} - \left( a - f_{\theta^{0}}(s,a) \right)^2 - 2 \left( f_{\theta^{0}}(s,a) - a \right) \left( f_{\theta^{t+1}_{n}}(s,a) - f_{\theta^{0}}(s,a) \right) \\
& \quad \left. - 2 \left( f_{\theta^{t+1}_{n}}(s,a) - f_{\theta^{0}}(s,a) \right)^2 \right] \\
&= \frac{1}{2 \sigma_{t+1}^{2}} \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ 2 \left( f_{\theta^{0}}(s,a) - a \right) \left( f_{\theta^{t+1}}(s,a) - f_{\theta^{t+1}_{n}}(s,a) \right) \right. \\
& \quad \left. + 2 \left( f_{\theta^{t+1}}(s,a) - f_{\theta^{0}}(s,a) \right)^{2} - 2 \left( f_{\theta^{t+1}_{n}}(s,a) - f_{\theta^{0}}(s,a) \right)^2 \right] \\
&\le \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \frac{f_{\theta^{0}}(s,a) - a}{\sigma_{t+1}^{2}} \left( f_{\theta^{t+1}}(s,a) - f_{\theta^{t+1}_{n}}(s,a) \right) \right] + \frac{R_{\theta}^{2}}{\sigma_{t+1}^{2}} \\
&\le \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \upsilon_{t+1}^{-1}(s,a) f_{\theta^{t+1}}(s,a) - \upsilon_{t+1}^{-1}(s,a) f_{\theta^{t+1}_{n}}(s,a) \right\vert \right] + \frac{R_{\theta}^{2}}{\sigma_{t+1}^{2}} \\
\le& 2 \mathbb{E}_{n \thicksim C} \left[ \sup \left\vert \upsilon_{t+1}^{-1}(s,a) \right\vert \tilde{\epsilon}_{n}^{t+1} \xi^{t+1}_{n} \right] + \beta_{t}^{-1} \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \sum_{i} q_{i} \left\vert Q^{w^{t}_{n}}(s,a) - Q^{w^{t}_{i}}(s,a) \right\vert \right] \nonumber \\
& + 2 \mathcal{O} \left( \sup \left\vert \upsilon_{t+1}^{-1}(s,a) \right\vert R_{\theta}^{3/2} m^{-1/4} \right) + \frac{R_{\theta}^{2}}{\sigma_{t+1}^{2}}.
\end{alignat}
\end{lemma}


\begin{lemma}
For energy-based policy,
\begin{alignat}{1}
-\Omega_{AC} &= -\sum_{s} \sum_{n} q_{n} \rho_{\pi^{\ast},n}(s) \left< \log \left( \pi^{\theta^{t+1}}(\cdot \vert s) / \pi^{\theta^{t+1}_{n}}(\cdot \vert s) \right), \pi^{\ast} \right> \\
&= \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \log \pi^{\theta_{n}^{t+1}}(s,a) - \log \pi^{\theta^{t+1}}(s,a) \right] \\
&= \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \tau^{-1}_{t+1} f_{\theta_{n}^{t+1}}(s,a) - \tau^{-1}_{t+1} f_{\theta^{t+1}}(s,a) \right] \\
&\le \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \tau_{t+1}^{-1} f_{\theta_{n}^{t+1}}(s,a) - \tau_{t+1}^{-1} f_{\theta^{t+1}}(s,a) \right\vert \right] \\
&\le 2 \mathbb{E}_{n \thicksim C} \left[ \tau_{t+1}^{-1} \epsilon^{t+1}_{n} \xi^{t+1}_{n} \right] + 2 \tau_{t+1}^{-1} \mathcal{O} \left( R_{\theta}^{3/2} m^{-1/4} \right).
\end{alignat}
For stochastic Gaussian policy,
\begin{alignat}{1}
-\Omega_{AC} &= -\sum_{s} \sum_{n} q_{n} \rho_{\pi^{\ast},n}(s) \left< \log \left( \pi^{\theta^{t+1}}(\cdot \vert s) / \pi^{\theta^{t+1}_{n}}(\cdot \vert s) \right), \pi^{\ast} \right> \\
&= \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \log \pi^{\theta_{n}^{t+1}} - \log \pi^{\theta^{t+1}} \right] \\
&= \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ - \frac{\left( a - f_{\theta^{t+1}_{n}}(s,a) \right)^2}{2 \sigma_{t+1}^{2}} - \log \sqrt{2 \pi} \sigma_{t+1} + \frac{\left( a - f_{\theta^{t+1}}(s,a) \right)^2}{2 \sigma_{t+1}^{2}} + \log \sqrt{2 \pi} \sigma_{t+1} \right] \\
&= \frac{1}{2 \sigma_{t+1}^{2}} \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left( a - f_{\theta^{t+1}}(s,a) \right)^2 - \left( a - f_{\theta^{t+1}_{n}}(s,a) \right)^2 \right] \\
&= \frac{1}{2 \sigma_{t+1}^{2}} \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left( a - f_{\theta^{0}}(s,a) \right)^2 + 2 \left( f_{\theta^{0}}(s,a) - a \right) \left( f_{\theta^{t+1}}(s,a) - f_{\theta^{0}}(s,a) \right) \right. \\
& \quad + 2 \left( f_{\theta^{t+1}}(s,a) - f_{\theta^{0}}(s,a) \right)^{2} - \left( a - f_{\theta^{0}}(s,a) \right)^2 - 2 \left( f_{\theta^{0}}(s,a) - a \right) \left( f_{\theta^{t+1}_{n}}(s,a) - f_{\theta^{0}}(s,a) \right) \\
& \quad \left. - 2 \left( f_{\theta^{t+1}_{n}}(s,a) - f_{\theta^{0}}(s,a) \right)^2 \right] \\
&= \frac{1}{2 \sigma_{t+1}^{2}} \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ 2 \left( f_{\theta^{0}}(s,a) - a \right) \left( f_{\theta^{t+1}}(s,a) - f_{\theta^{t+1}_{n}}(s,a) \right) \right. \\
& \quad \left. + 2 \left( f_{\theta^{t+1}}(s,a) - f_{\theta^{0}}(s,a) \right)^{2} - 2 \left( f_{\theta^{t+1}_{n}}(s,a) - f_{\theta^{0}}(s,a) \right)^2 \right] \\
&\le \frac{1}{\sigma_{t+1}^{2}} \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left( f_{\theta^{0}}(s,a) - a \right) \left( f_{\theta^{t+1}}(s,a) - f_{\theta^{t+1}_{n}}(s,a) \right) \right] + \frac{R_{\theta}^{2}}{\sigma_{t+1}^{2}} \\
&\le \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \left( \upsilon^{-1}_{t+1}(s,a) f_{\theta^{t+1}}(s,a) - \upsilon^{-1}_{t+1}(s,a) f_{\theta^{t+1}_{n}}(s,a) \right\vert \right) \right] + \frac{R_{\theta}^{2}}{\sigma_{t+1}^{2}} \\
\le& 2 \mathbb{E}_{n \thicksim C} \left[ \sup \left\vert \upsilon_{t+1}^{-1}(s,a) \right\vert \tilde{\epsilon}_{n}^{t+1} \xi^{t+1}_{n} \right] + 2 \mathcal{O} \left( \sup \left\vert \upsilon_{t+1}^{-1}(s,a) \right\vert R_{\theta}^{3/2} m^{-1/4} \right) + \frac{R_{\theta}^{2}}{\sigma_{t+1}^{2}}.
\end{alignat}
\end{lemma}
\end{proof}

\begin{alignat}{1}
& \left\vert \mathbb{E}_{s \thicksim \rho_{\pi^{\ast},n}} \left[ \left< \log \left( \pi^{\theta^{t+1}_{n}}(\cdot \vert s) / \pi^{t+1}_{n}(\cdot \vert s) \right), \pi^{\ast}(\cdot \vert s) - \pi^{\theta^{t}}(\cdot \vert s) \right> \right] \right\vert \nonumber \\
=& \left\vert \mathbb{E}_{s \thicksim \rho_{\pi^{\ast},n}} \left[ \left< \log \pi^{\theta^{t+1}_{n}}(\cdot \vert s) - \left( \beta_{t}^{-1} Q^{\pi^{\theta^{t}}}(s,\cdot) + \log \pi^{\theta^{t}}(\cdot \vert s) \right), \pi^{\ast}(\cdot \vert s) - \pi^{\theta^{t}}(\cdot \vert s) \right> \right] \right\vert \\
=& \left\vert \mathbb{E}_{s \thicksim \rho_{\pi^{\ast},n}} \left[ \left< \log \pi^{\theta^{t+1}_{n}}(\cdot \vert s) - \left( \beta_{t}^{-1} Q^{w^{t}}(s,\cdot) + \log \pi^{\theta^{t}}(\cdot \vert s) \right), \pi^{\ast}(\cdot \vert s) - \pi^{\theta^{t}}(\cdot \vert s) \right> \right] \right. \nonumber \\
& \left. + \mathbb{E}_{s \thicksim \rho_{\pi^{\ast},n}} \left[ \left< \beta_{t}^{-1} Q^{\pi^{\theta^{t}}}(s,\cdot) - \beta_{t}^{-1} Q^{w^{t}}(s,\cdot), \pi^{\ast}(\cdot \vert s) - \pi^{\theta^{t}}(\cdot \vert s) \right> \right] \right\vert \\
=& \left\vert \int_{\mathcal{S}} \left< \log \pi^{\theta^{t+1}_{n}}(\cdot \vert s) - \left( \beta_{t}^{-1} Q^{w^{t}}(s,\cdot) + \log \pi^{\theta^{t}}(\cdot \vert s) \right), \pi^{\theta^{t}}(\cdot \vert s) \rho_{\pi^{\theta^{t}},n}(s) \left( \frac{\pi^{\ast}(\cdot \vert s)}{\pi^{\theta^{t}}(\cdot \vert s)} - \frac{\pi^{\theta^{t}}(\cdot \vert s)}{\pi^{\theta^{t}}(\cdot \vert s)} \right) \right> \cdot \frac{\rho_{\pi^{\ast},n}(s)}{\rho_{\pi^{\theta^{t}},n}(s)} \mathrm{d} s \right. \nonumber \\
& \left. + \int_{\mathcal{S}} \left< \beta_{t}^{-1} Q^{\pi^{\theta^{t}}}(s,\cdot) - \beta_{t}^{-1} Q^{w^{t}}(s,\cdot), \pi^{\theta^{t}}(\cdot \vert s) \rho_{\pi^{\theta^{t}},n}(s) \left( \frac{\pi^{\ast}(\cdot \vert s)}{\pi^{\theta^{t}}(\cdot \vert s)} - \frac{\pi^{\theta^{t}}(\cdot \vert s)}{\pi^{\theta^{t}}(\cdot \vert s)} \right) \right> \cdot \frac{\rho_{\pi^{\ast},n}(s)}{\rho_{\pi^{\theta^{t}},n}(s)} \mathrm{d} s \right\vert \\
\le& \left\vert \int_{\mathcal{S}} \left< \log \pi^{\theta^{t+1}_{n}}(\cdot \vert s) - \left( \beta_{t}^{-1} Q^{w^{t}}(s,\cdot) + \log \pi^{\theta^{t}}(\cdot \vert s) \right), \pi^{\theta^{t}}(\cdot \vert s) \rho_{\pi^{\theta^{t}},n}(s) \left( \frac{\pi^{\ast}(\cdot \vert s)}{\pi^{\theta^{t}}(\cdot \vert s)} - \frac{\pi^{\theta^{t}}(\cdot \vert s)}{\pi^{\theta^{t}}(\cdot \vert s)} \right) \right> \cdot \frac{\rho_{\pi^{\ast},n}(s)}{\rho_{\pi^{\theta^{t}},n}(s)} \mathrm{d} s \right\vert \nonumber \\
& + \left\vert \int_{\mathcal{S}} \left< \beta_{t}^{-1} Q^{\pi^{\theta^{t}}}(s,\cdot) - \beta_{t}^{-1} Q^{w^{t}}(s,\cdot), \pi^{\theta^{t}}(\cdot \vert s) \rho_{\pi^{\theta^{t}},n}(s) \left( \frac{\pi^{\ast}(\cdot \vert s)}{\pi^{\theta^{t}}(\cdot \vert s)} - \frac{\pi^{\theta^{t}}(\cdot \vert s)}{\pi^{\theta^{t}}(\cdot \vert s)} \right) \right> \cdot \frac{\rho_{\pi^{\ast},n}(s)}{\rho_{\pi^{\theta^{t}},n}(s)} \mathrm{d} s \right\vert \\
\le& \left\vert \int_{\mathcal{S} \times \mathcal{A}} \left( \log \pi^{\theta^{t+1}_{n}}(\cdot \vert s) - \left( \beta_{t}^{-1} Q^{w^{t}}(s,\cdot) + \log \pi^{\theta^{t}}(\cdot \vert s) \right) \right) \cdot \left( \frac{\rho_{\pi^{\ast},n}(s) \pi^{\ast}(\cdot \vert s)}{\rho_{\pi^{\theta^{t}},n}(s) \pi^{\theta^{t}}(\cdot \vert s)} - \frac{\rho_{\pi^{\ast},n}(s)}{\rho_{\pi^{\theta^{t}},n}(s)} \right) \mathrm{d} \rho_{\pi^{\theta^{t}}}(s) \pi^{\theta^{t}}(a \vert s) \right\vert \nonumber \\
& + \left\vert \int_{\mathcal{S} \times \mathcal{A}} \left( \beta_{t}^{-1} Q^{\pi^{\theta^{t}}}(s,\cdot) - \beta_{t}^{-1} Q^{w^{t}}(s,\cdot) \right) \cdot \left( \frac{\rho_{\pi^{\ast},n}(s) \pi^{\ast}(\cdot \vert s)}{\rho_{\pi^{\theta^{t}},n}(s) \pi^{\theta^{t}}(\cdot \vert s)} - \frac{\rho_{\pi^{\ast},n}(s)}{\rho_{\pi^{\theta^{t}},n}(s)} \right) \mathrm{d} \rho_{\pi^{\theta^{t}}}(s) \pi^{\theta^{t}}(a \vert s) \right\vert \\
\le& \mathbb{E}_{s \thicksim \rho_{\pi^{\theta^{t},n}, a \thicksim \pi^{\theta^{t}}}} \left[ \log \pi^{\theta^{t+1}_{n}}(\cdot \vert s) - \left( \beta_{t}^{-1} Q^{w^{t}}(s,\cdot) + \log \pi^{\theta^{t}}(\cdot \vert s) \right)^{2} \right]^{1/2} \mathbb{E}_{s \thicksim \rho_{\pi^{\theta^{t},n}, a \thicksim \pi^{\theta^{t}}}} \left[ \left( \frac{\rho_{\pi^{\ast},n}(s) \pi^{\ast}(\cdot \vert s)}{\rho_{\pi^{\theta^{t}},n}(s) \pi^{\theta^{t}}(\cdot \vert s)} - \frac{\rho_{\pi^{\ast},n}(s)}{\rho_{\pi^{\theta^{t}},n}(s)} \right)^{2} \right]^{1/2} \nonumber \\
& + \mathbb{E}_{s \thicksim \rho_{\pi^{\theta^{t},n}, a \thicksim \pi^{\theta^{t}}}} \left[ \left( \beta_{t}^{-1} Q^{\pi^{\theta^{t}}}(s,\cdot) - \beta_{t}^{-1} Q^{w^{t}}(s,\cdot) \right)^{2} \right]^{1/2} \mathbb{E}_{s \thicksim \rho_{\pi^{\theta^{t},n}, a \thicksim \pi^{\theta^{t}}}} \left[ \left( \frac{\rho_{\pi^{\ast},n}(s) \pi^{\ast}(\cdot \vert s)}{\rho_{\pi^{\theta^{t}},n}(s) \pi^{\theta^{t}}(\cdot \vert s)} - \frac{\rho_{\pi^{\ast},n}(s)}{\rho_{\pi^{\theta^{t}},n}(s)} \right)^{2} \right]^{1/2} \\
\le& \sup \left\vert c_{t+1}^{-1}(s,a) \right\vert \epsilon^{t+1}_{n} \psi^{t}_{n} + \beta_{t+1}^{-1} \dot{\epsilon}^{t+1}_{n} \psi^{t}_{n},
\end{alignat}
where $c_{t}(s,a) = \tau_{t}$ for Softmax policy and $c_{t}(s,a) = \upsilon_{t}(s,a)$ for Gaussian policy.

\section{Proof of Lemma \ref{lemma:stepwise_energy_difference}\label{proof:lemma:stepwise_energy_difference}}

\begin{proof}
For Softmax policy, we have
\begin{alignat}{1}
& \mathbb{E}_{s \thicksim \rho_{\pi^{\ast},n}} \left[ \left\Vert \tau_{t+1}^{-1} f_{\theta^{t+1}_{n}}(s,\cdot) - \tau_{t}^{-1} f_{\theta^{t}}(s,\cdot) \right\Vert_{\infty}^{2} \right] \nonumber \\
=& \mathbb{E}_{s \thicksim \rho_{\pi^{\ast},n}} \left[ \left\vert \tau_{t+1}^{-1} f_{\theta^{t+1}_{n}}(s,a_{\max}(s)) - \tau_{t}^{-1} f_{\theta^{t}}(s,a_{\max}(s)) \right\vert^{2} \right] \\
=& \mathbb{E}_{s \thicksim \rho_{\pi^{\ast},n}} \left[ \left( \vert \tau_{t+1}^{-1} \vert \vert f_{\theta^{t+1}_{n}}(s,a_{\max}(s)) - f_{\theta^{t}}(s,a_{\max}(s)) \vert - \vert f_{\theta^{t}}(s,a_{\max}(s)) \vert \vert \tau_{t+1}^{-1} - \tau_{t}^{-1} \vert \right)^{2} \right] \\
\le& \mathbb{E}_{s \thicksim \rho_{\pi^{\ast},n}} \left[ 2 \vert \tau_{t+1}^{-1} \vert^{2} \vert f_{\theta^{t+1}_{n}}(s,a_{\max}(s)) - f_{\theta^{t}}(s,a_{\max}(s)) \vert^{2} + 2 \vert f_{\theta^{t}}(s,a_{\max}(s)) \vert^{2} \vert \tau_{t+1}^{-1} - \tau_{t}^{-1} \vert^{2} \right] \\
\le& \mathbb{E}_{s \thicksim \rho_{\pi^{\ast},n}} \left[ 8 ( \tau_{t+1}^{-1} )^{2} R_{\theta}^{2} + 4 \left( \max_{a \in \mathcal{A}} f_{\theta^{0}}^{2}(s,a) + R_{\theta}^{2} \right) ( \tau_{t+1}^{-1} - \tau_{t}^{-1} )^{2} \right],
\end{alignat}
where the first equality and the first inequality follow from the fact that $(a + b)^{2} \le 2a^{2} + 2b^{2}$ and $ab - cd = a(b-c) + c(a-d)$, respectively. The second inequality follows from Lemma \ref{lemma:bounded_by_r} and the fact that $\left( f_{\theta^{t}}(s,a) \le f_{\theta^{0}}(s,a) +2 R_{\theta}^{2} \right)^{2}$, which is due to the 1-Lipschitz continuity of $f_{\theta}$ w.r.t. $\theta$.

For Gaussian policy, by Lemma \ref{lemma:taylor_expansion}, we have
\begin{alignat}{1}
& \mathbb{E}_{s \thicksim \rho_{\pi^{\ast},n}} \left[ \left\Vert - \frac{(a - f_{\theta_{n}^{t+1}})^{2}}{2 \sigma_{t+1}^{2}} - \log \sigma_{t+1} + \frac{(a - f_{\theta^{t}})^{2}}{2 \sigma_{t}^{2}} + \log \sigma_{t} \right\Vert_{\infty}^{2} \right] \nonumber \\
=& \mathbb{E}_{s \thicksim \rho_{\pi^{\ast},n}} \left[ \left( - \frac{(a_{\max}(s) - f_{\theta^{0}})^{2}}{2 \sigma_{t+1}^{2}} - \frac{1}{\sigma_{t+1}^{2}} ( f_{\theta^{0}} - a_{\max}(s) ) ( f_{\theta_{n}^{t+1}} - f_{\theta^{0}} ) - \frac{1}{2 \sigma_{t+1}^{2}} ( f_{\theta^{t+1}_{n}} - f_{\theta^{0}} )^{2} \right. \right. \nonumber \\
& \left. \left. + \frac{(a_{\max}(s) - f_{\theta^{0}})^{2}}{2 \sigma_{t}^{2}} + \frac{1}{\sigma_{t}^{2}} ( f_{\theta^{0}} - a_{\max}(s) ) ( f_{\theta^{t}} - f_{\theta^{0}} ) + \frac{1}{2 \sigma_{t}^{2}} ( f_{\theta^{t}} - f_{\theta^{0}} )^{2} + \log \frac{\sigma_{t}}{\sigma_{t+1}} \right)^{2} \right] \\
=& \mathbb{E}_{s \thicksim \rho_{\pi^{\ast},n}} \left[ \left( \frac{1}{\sigma_{t}^{2}} ( f_{\theta^{0}} - a_{\max}(s) ) f_{\theta^{t}} - \frac{1}{\sigma_{t+1}^{2}} ( f_{\theta^{0}} - a_{\max}(s) ) f_{\theta_{n}^{t+1}} + \frac{1}{\sigma_{t+1}^{2}} ( f_{\theta^{0}} - a_{\max}(s) ) f_{\theta^{0}} - \frac{1}{\sigma_{t}^{2}} ( f_{\theta^{0}} - a_{\max}(s) )  f_{\theta^{0}} \right. \right. \nonumber \\
& \left. \left. + \frac{(a_{\max}(s) - f_{\theta^{0}})^{2}}{2 \sigma_{t}^{2}} - \frac{(a_{\max}(s) - f_{\theta^{0}})^{2}}{2 \sigma_{t+1}^{2}} + \frac{1}{2 \sigma_{t}^{2}} ( f_{\theta^{t}} - f_{\theta^{0}} )^{2} - \frac{1}{2 \sigma_{t+1}^{2}} ( f_{\theta^{t+1}_{n}} - f_{\theta^{0}} )^{2} + \log \frac{\sigma_{t}}{\sigma_{t+1}} \right)^{2} \right] \\
=& \mathbb{E}_{s \thicksim \rho_{\pi^{\ast},n}} \left[ \left( \upsilon_{t+1}^{-1}(s,a_{\max}(s)) f_{\theta^{t+1}_{n}} - \upsilon_{t}^{-1}(s,a_{\max}(s)) f_{\theta^{t}} + \frac{1}{2 \sigma_{t}^{2}} ( f_{\theta^{t}} - f_{\theta^{0}} )^{2} - \frac{1}{2 \sigma_{t+1}^{2}} ( f_{\theta^{t+1}_{n}} - f_{\theta^{0}} )^{2} + \log \frac{\sigma_{t}}{\sigma_{t+1}} \right. \right. \nonumber \\
& \left. \left. + \left( \frac{f_{\theta^{0}}}{\sigma_{t+1}^{2}} - \frac{f_{\theta^{0}}}{\sigma_{t}^{2}} - \frac{f_{\theta^{0}} - a_{\max}(s)}{2 \sigma
_{t+1}^{2}} + \frac{f_{\theta^{0}} - a_{\max}(s)}{2 \sigma_{t}^{2}} \right) ( f_{\theta^{0}} - a_{\max}(s) ) \right)^{2} \right] \\
\le& \mathbb{E}_{s \thicksim \rho_{\pi^{\ast},n}} \left[ 3 \left( \upsilon_{t+1}^{-1}(s,a_{\max}(s)) f_{\theta^{t+1}_{n}} - \upsilon_{t}^{-1}(s,a_{\max}(s)) f_{\theta^{t}} \right)^{2} + 3 \left( \frac{1}{2 \sigma_{t}^{2}} ( f_{\theta^{t}} - f_{\theta^{0}} )^{2} - \frac{1}{2 \sigma_{t+1}^{2}} ( f_{\theta^{t+1}_{n}} - f_{\theta^{0}} )^{2} \right)^{2} \right. \nonumber \\
& \left. + 3 \left( \log \frac{\sigma_{t}}{\sigma_{t+1}} + \frac{1}{2} \left( \frac{1}{\sigma_{t+1}^{2}} - \frac{1}{\sigma_{t}^{2}} \right) ( f_{\theta^{0}}^{2} - a_{\max}(s)^{2} ) \right)^{2} \right] \\
\le& 3 \mathbb{E}_{s \thicksim \rho_{\pi^{\ast},n}} \left[ \left( \upsilon_{t+1}^{-1}(s,a_{\max}(s)) f_{\theta^{t+1}_{n}} - \upsilon_{t}^{-1}(s,a_{\max}(s)) f_{\theta^{t}} \right)^{2} \right] + 3 \mathbb{E}_{s \thicksim \rho_{\pi^{\ast},n}} \left[ \max_{a \in \mathcal{A}} \left( \log \frac{\sigma_{t}}{\sigma_{t+1}} + \frac{1}{2} \left( \frac{1}{\sigma_{t+1}^{2}} - \frac{1}{\sigma_{t}^{2}} \right) ( f_{\theta^{0}}^{2} - a^{2} ) \right)^{2} \right] \nonumber \\
& + \frac{3 R_{\theta}^{4}}{4 \sigma_{t+1}^{4}} \\
\le& \mathbb{E}_{s \thicksim \rho_{\pi^{\ast},n}} \left[ \max_{a \in \mathcal{A}} \left( 24 ( \upsilon_{t+1}^{-1}(s, a) )^{2} R_{\theta}^{2} + 12 \left( f_{\theta^{0}}^{2}(s,a) + R_{\theta}^{2} \right) ( \upsilon_{t+1}^{-1}(s, a) - \upsilon_{t}^{-1}(s, a) )^{2} \right) \right] \nonumber \\
& + 3 \mathbb{E}_{s \thicksim \rho_{\pi^{\ast},n}} \left[ \max_{a \in \mathcal{A}} \left( \log \frac{\sigma_{t}}{\sigma_{t+1}} + \frac{1}{2} \left( \frac{1}{\sigma_{t+1}^{2}} - \frac{1}{\sigma_{t}^{2}} \right) ( f_{\theta^{0}}^{2} - a^{2} ) \right)^{2} \right] + \frac{3 R_{\theta}^{4}}{4 \sigma_{t+1}^{4}}
\end{alignat}
\end{proof}


\section{Proof of Lemma \ref{lemma:aggregation_error}\label{proof:lemma:aggregation_error}}

\begin{proof}

\begin{lemma}
For the baseline with Softmax policy,



\begin{alignat}{1}
& \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \tau_{t+1}^{-1} f_{\theta_{n}^{t+1}}(s,a) - \tau_{t+1}^{-1} f_{\theta^{t+1}}(s,a) \right\vert \right] \\
\le& \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \tau_{t+1}^{-1} f_{\theta_{n}^{t+1}}(s,a) - \tau_{t+1}^{-1} f_{\theta^{t+1}}^{0}(s,a) \right\vert + \left\vert \tau_{t+1}^{-1} f_{\theta^{t+1}}^{0}(s,a) - \tau_{t+1}^{-1} f_{\theta^{t+1}}(s,a) \right\vert \right] \\
=& \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \tau_{t+1}^{-1} f_{\theta_{n}^{t+1}}(s,a) - \tau_{t+1}^{-1} f_{\theta^{t+1}}^{0}(s,a) \right\vert \right] + \mathcal{O} \left( \tau_{t+1}^{-1} R_{\theta}^{3/2} m^{-1/4} \right) \\
=& \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \tau_{t+1}^{-1} f_{\theta_{n}^{t+1}}(s,a) - \sum_{i} q_{i} \tau_{t+1}^{-1} f_{\theta^{t+1}_{i}}^{0}(s,a) \right\vert \right] + \mathcal{O} \left( \tau_{t+1}^{-1} R_{\theta}^{3/2} m^{-1/4} \right) \\
\le& \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \tau_{t+1}^{-1} f_{\theta_{n}^{t+1}}(s,a) - \sum_{i} q_{i} \tau_{t+1}^{-1} f_{\theta^{t+1}_{i}}(s,a) \right\vert + \left\vert \sum_{i} q_{i} \tau_{t+1}^{-1} f_{\theta^{t+1}_{i}}(s,a) - \sum_{i} q_{i} \tau_{t+1}^{-1} f_{\theta^{t+1}_{i}}^{0}(s,a) \right\vert \right] \nonumber \\
& + \mathcal{O} \left( \tau_{t+1}^{-1} R_{\theta}^{3/2} m^{-1/4} \right) \\
\le& \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \tau_{t+1}^{-1} f_{\theta_{n}^{t+1}}(s,a) - \sum_{i} q_{i} \tau_{t+1}^{-1} f_{\theta^{t+1}_{i}}(s,a) \right\vert \right] + 2 \mathcal{O} \left( \tau_{t+1}^{-1} R_{\theta}^{3/2} m^{-1/4} \right) \\
\le& \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \tau_{t+1}^{-1} f_{\theta_{n}^{t+1}}(s,a) - \left( \beta_{t}^{-1} Q^{w^{t}_{n}}(s,a) + \tau_{t}^{-1} f_{\theta^{t}}(s,a) \right) \right\vert \right. \nonumber \\
& \left. + \sum_{i} q_{i} \left\vert \left( \beta_{t}^{-1} Q^{w^{t}_{n}}(s,a) + \tau_{t}^{-1} f_{\theta^{t}}(s,a) \right) - \left( \beta_{t}^{-1} Q^{w^{t}_{i}}(s,a) + \tau_{t}^{-1} f_{\theta^{t}}(s,a) \right) \right\vert \right. \nonumber \\
& \left. + \sum_{i} q_{i} \left\vert \tau_{t+1}^{-1} f_{\theta_{i}^{t+1}}(s,a) - \left( \beta_{t}^{-1} Q^{w^{t}_{i}}(s,a) + f_{\theta^{t}}(s,a) \right) \right\vert \right] + 2 \mathcal{O} \left( \tau_{t+1}^{-1} R_{\theta}^{3/2} m^{-1/4} \right) \\
=& \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \tau_{t+1}^{-1} f_{\theta_{n}^{t+1}}(s,a) - \left( \beta_{t}^{-1} Q^{w^{t}_{n}}(s,a) + \tau_{t}^{-1} f_{\theta^{t}}(s,a) \right) \right\vert \right. \nonumber \\
& \left. + \beta_{t}^{-1} \sum_{i} q_{i} \left\vert Q^{w^{t}_{n}}(s,a) - Q^{w^{t}_{i}}(s,a) \right\vert \right. \nonumber \\
& \left. + \sum_{i} q_{i} \left\vert \tau_{t+1}^{-1} f_{\theta_{i}^{t+1}}(s,a) - \left( \beta_{t}^{-1} Q^{w^{t}_{i}}(s,a) + \tau_{t}^{-1} f_{\theta^{t}}(s,a) \right) \right\vert \right] + 2 \mathcal{O} \left( \tau_{t+1}^{-1} R_{\theta}^{3/2} m^{-1/4} \right) \\
\le& 2 \mathbb{E}_{n \thicksim C} \left[ \tau_{t+1}^{-1} \epsilon^{t+1}_{n} \xi^{t+1}_{n} \right] + \beta_{t}^{-1} \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \sum_{i} q_{i} \left\vert Q^{w^{t}_{n}}(s,a) - Q^{w^{t}_{i}}(s,a) \right\vert \right] + 2 \mathcal{O} \left( \tau_{t+1}^{-1} R_{\theta}^{3/2} m^{-1/4} \right).
\end{alignat}
For CA and Gaussian policy,
\begin{alignat}{1}
& \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \upsilon_{t+1}^{-1}(s,a) f_{\theta_{n}^{t+1}}(s,a) - \upsilon_{t+1}^{-1}(s,a) f_{\theta^{t+1}}(s,a) \right\vert \right] \\
\le& \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \upsilon_{t+1}^{-1}(s,a) f_{\theta_{n}^{t+1}}(s,a) - \upsilon_{t+1}^{-1}(s,a) f_{\theta^{t+1}}^{0}(s,a) \right\vert + \left\vert \upsilon_{t+1}^{-1}(s,a) f_{\theta^{t+1}}^{0}(s,a) - \upsilon_{t+1}^{-1}(s,a) f_{\theta^{t+1}}(s,a) \right\vert \right] \\
\le& \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \upsilon_{t+1}^{-1} f_{\theta_{n}^{t+1}}(s,a) - \upsilon_{t+1}^{-1} f_{\theta^{t+1}}^{0}(s,a) \right\vert \right] + \mathcal{O} \left( \sup \left\vert \upsilon_{t+1}^{-1}(s,a) \right\vert R_{\theta}^{3/2} m^{-1/4} \right) \\
=& \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \upsilon_{t+1}^{-1}(s,a) f_{\theta_{n}^{t+1}}(s,a) - \sum_{i} q_{i} \upsilon_{t+1}^{-1}(s,a) f_{\theta^{t+1}_{i}}^{0}(s,a) \right\vert \right] + \mathcal{O} \left( \sup \left\vert \upsilon_{t+1}^{-1}(s,a) \right\vert R_{\theta}^{3/2} m^{-1/4} \right) \\
\le& \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \upsilon_{t+1}^{-1}(s,a) f_{\theta_{n}^{t+1}}(s,a) - \sum_{i} q_{i} \upsilon_{t+1}^{-1}(s,a) f_{\theta^{t+1}_{i}}(s,a) \right\vert \right. \nonumber \\
& + \left. \left\vert \sum_{i} q_{i} \upsilon_{t+1}^{-1}(s,a) f_{\theta^{t+1}_{i}}(s,a) - \sum_{i} q_{i} \upsilon_{t+1}^{-1}(s,a) f_{\theta^{t+1}_{i}}^{0}(s,a) \right\vert \right]  \nonumber \\
& + \mathcal{O} \left( \sup \left\vert \upsilon_{t+1}^{-1}(s,a) \right\vert R_{\theta}^{3/2} m^{-1/4} \right) \\
\le& \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \upsilon_{t+1}^{-1}(s,a) f_{\theta_{n}^{t+1}}(s,a) - \sum_{i} q_{i} \upsilon_{t+1}^{-1}(s,a) f_{\theta^{t+1}_{i}}(s,a) \right\vert \right] + 2 \mathcal{O} \left( \sup \left\vert \upsilon_{t+1}^{-1}(s,a) \right\vert R_{\theta}^{3/2} m^{-1/4} \right) \\
\le& \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \upsilon_{t+1}^{-1}(s,a) f_{\theta_{n}^{t+1}}(s,a) - \left( \beta_{t}^{-1} Q^{w^{t}_{n}}(s,a) + \upsilon_{t}(s,a)^{-1} f_{\theta^{t}}(s,a) \right) \right\vert \right. \nonumber \\
& \left. + \sum_{i} q_{i} \left\vert \left( \beta_{t}^{-1} Q^{w^{t}_{n}}(s,a) + \upsilon_{t}^{-1}(s,a) f_{\theta^{t}}(s,a) \right) - \left( \beta_{t}^{-1} Q^{w^{t}_{i}}(s,a) + \upsilon_{t}^{-1}(s,a) f_{\theta^{t}}(s,a) \right) \right\vert \right. \nonumber \\
& \left. + \sum_{i} q_{i} \left\vert \upsilon_{t+1}^{-1}(s,a) f_{\theta_{i}^{t+1}}(s,a) - \left( \beta_{t}^{-1} Q^{w^{t}_{i}}(s,a) + 
\upsilon_{t}^{-1}(s,a) f_{\theta^{t}}(s,a) \right) \right\vert \right] + 2 \mathcal{O} \left( \sup \left\vert \upsilon_{t+1}^{-1}(s,a) \right\vert R_{\theta}^{3/2} m^{-1/4} \right) \\
=& \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \upsilon_{t+1}^{-1}(s,a) f_{\theta_{n}^{t+1}}(s,a) - \left( \beta_{t}^{-1} Q^{w^{t}_{n}}(s,a) + \upsilon_{t}^{-1}(s,a) f_{\theta^{t}}(s,a) \right) \right\vert \right. \nonumber \\
& \left. + \beta_{t}^{-1} \sum_{i} q_{i} \left\vert Q^{w^{t}_{n}}(s,a) - Q^{w^{t}_{i}}(s,a) \right\vert \right. \nonumber \\
& \left. + \sum_{i} q_{i} \left\vert \upsilon_{t+1}^{-1}(s,a) f_{\theta_{i}^{t+1}}(s,a) - \left( \beta_{t}^{-1} Q^{w^{t}_{i}}(s,a) + \upsilon_{t}^{-1}(s,a) f_{\theta^{t}}(s,a) \right) \right\vert \right] + 2 \mathcal{O} \left( \sup \left\vert \upsilon_{t+1}^{-1}(s,a) \right\vert R_{\theta}^{3/2} m^{-1/4} \right) \\
=& \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \upsilon_{t+1}^{-1}(s,a) f_{\theta_{n}^{t+1}}(s,a) - \left( \beta_{t}^{-1} Q^{w^{t}_{n}}(s,a) + \upsilon_{t}^{-1}(s,a) f_{\theta^{t}}(s,a) \right) \right\vert \right. \nonumber \\
& \left. + \beta_{t}^{-1} \sum_{i} q_{i} \left\vert Q^{w^{t}_{n}}(s,a) - Q^{w^{t}_{i}}(s,a) \right\vert \right. \nonumber \\
& \left. + \sum_{i} q_{i} \left\vert \upsilon_{t+1}^{-1}(s,a) f_{\theta_{i}^{t+1}}(s,a) - \left( \beta_{t}^{-1} Q^{w^{t}_{i}}(s,a) + \upsilon_{t}^{-1}(s,a) f_{\theta^{t}}(s,a) \right) \right\vert \right] + 2 \mathcal{O} \left( \sup \left\vert \upsilon_{t+1}^{-1}(s,a) \right\vert R_{\theta}^{3/2} m^{-1/4} \right) \\
\le& 2 \mathbb{E}_{n \thicksim C} \left[ \sup \left\vert \upsilon_{t+1}^{-1}(s,a) \right\vert \tilde{\epsilon}_{n}^{t+1} \xi^{t+1}_{n} \right] + \beta_{t}^{-1} \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \sum_{i} q_{i} \left\vert Q^{w^{t}_{n}}(s,a) - Q^{w^{t}_{i}}(s,a) \right\vert \right] + 2 \mathcal{O} \left( \sup \left\vert \upsilon_{t+1}^{-1}(s,a) \right\vert R_{\theta}^{3/2} m^{-1/4} \right).
\end{alignat}
For AC and Softmax policy,
\begin{alignat}{1}
& \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \tau_{t+1}^{-1} f_{\theta_{n}^{t+1}}(s,a) - \tau_{t+1}^{-1} f_{\theta^{t+1}}(s,a) \right\vert \right] \\
\le& \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \tau_{t+1}^{-1} f_{\theta_{n}^{t+1}}(s,a) - \tau_{t+1}^{-1} f_{\theta^{t+1}}^{0}(s,a) \right\vert + \left\vert \tau_{t+1}^{-1} f_{\theta^{t+1}}^{0}(s,a) - \tau_{t+1}^{-1} f_{\theta^{t+1}}(s,a) \right\vert \right] \\
=& \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \tau_{t+1}^{-1} f_{\theta_{n}^{t+1}}(s,a) - \tau_{t+1}^{-1} f_{\theta^{t+1}}^{0}(s,a) \right\vert \right] + \mathcal{O} \left( \tau_{t+1}^{-1} R_{\theta}^{3/2} m^{-1/4} \right) \\
=& \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \tau_{t+1}^{-1} f_{\theta_{n}^{t+1}}(s,a) - \sum_{i} q_{i} \tau_{t+1}^{-1} f_{\theta^{t+1}_{i}}^{0}(s,a) \right\vert \right] + \mathcal{O} \left( \tau_{t+1}^{-1} R_{\theta}^{3/2} m^{-1/4} \right) \\
\le& \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \tau_{t+1}^{-1} f_{\theta_{n}^{t+1}}(s,a) - \sum_{i} q_{i} \tau_{t+1}^{-1} f_{\theta^{t+1}_{i}}(s,a) \right\vert + \left\vert \sum_{i} q_{i} \tau_{t+1}^{-1} f_{\theta^{t+1}_{i}}(s,a) - \sum_{i} q_{i} \tau_{t+1}^{-1} f_{\theta^{t+1}_{i}}^{0}(s,a) \right\vert \right] \nonumber \\
& + \mathcal{O} \left( \tau_{t+1}^{-1} R_{\theta}^{3/2} m^{-1/4} \right) \\
\le& \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \tau_{t+1}^{-1} f_{\theta_{n}^{t+1}}(s,a) - \sum_{i} q_{i} \tau_{t+1}^{-1} f_{\theta^{t+1}_{i}}(s,a) \right\vert \right] + 2 \mathcal{O} \left( \tau_{t+1}^{-1} R_{\theta}^{3/2} m^{-1/4} \right) \\
\le& \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \tau_{t+1}^{-1} f_{\theta_{n}^{t+1}}(s,a) - \left( \beta_{t}^{-1} Q^{w^{t}}(s,a) + \tau_{t}^{-1} f_{\theta^{t}}(s,a) \right) \right\vert \right. \\
& \left. + \sum_{i} q_{i} \left\vert \left( \beta_{t}^{-1} Q^{w^{t}}(s,a) + \tau_{t}^{-1} f_{\theta^{t}}(s,a) \right) - \left( \beta_{t}^{-1} Q^{w^{t}}(s,a) + \tau_{t}^{-1} f_{\theta^{t}}(s,a) \right) \right\vert \right. \\
& \left. + \sum_{i} q_{i} \left\vert \tau_{t+1}^{-1} f_{\theta_{i}^{t+1}}(s,a) - \left( \beta_{t}^{-1} Q^{w^{t}}(s,a) + \tau_{t}^{-1} f_{\theta^{t}}(s,a) \right) \right\vert \right] + 2 \mathcal{O} \left( \tau_{t+1}^{-1} R_{\theta}^{3/2} m^{-1/4} \right) \\
=& \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \tau_{t+1}^{-1} f_{\theta_{n}^{t+1}}(s,a) - \left( \beta_{t}^{-1} Q^{w^{t}}(s,a) + \tau_{t}^{-1} f_{\theta^{t}}(s,a) \right) \right\vert \right. \\
& \left. + \beta_{t}^{-1} \sum_{i} q_{i} \left\vert Q^{w^{t}}(s,a) - Q^{w^{t}}(s,a) \right\vert \right. \\
& \left. + \sum_{i} q_{i} \left\vert \tau_{t+1}^{-1} f_{\theta_{i}^{t+1}}(s,a) - \left( \beta_{t}^{-1} Q^{w^{t}}(s,a) + \tau_{t}^{-1} f_{\theta^{t}}(s,a) \right) \right\vert \right] + 2 \mathcal{O} \left( R_{\theta}^{3/2} m^{-1/4} \right) \\
\le& 2 \mathbb{E}_{n \thicksim C} \left[ \tau_{t+1}^{-1} \epsilon^{t+1}_{n} \xi^{t+1}_{n} \right] + 2 \mathcal{O} \left( \tau_{t+1}^{-1} R_{\theta}^{3/2} m^{-1/4} \right).
\end{alignat}
For AC and Gaussian policy,
\begin{alignat}{1}
& \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \upsilon_{t+1}^{-1}(s,a) f_{\theta_{n}^{t+1}}(s,a) - \upsilon_{t+1}^{-1}(s,a) f_{\theta^{t+1}}(s,a) \right\vert \right] \\
\le& \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \upsilon_{t+1}^{-1}(s,a) f_{\theta_{n}^{t+1}}(s,a) - \upsilon_{t+1}^{-1}(s,a) f_{\theta^{t+1}}^{0}(s,a) \right\vert + \left\vert \upsilon_{t+1}^{-1}(s,a) f_{\theta^{t+1}}^{0}(s,a) - \upsilon_{t+1}^{-1}(s,a) f_{\theta^{t+1}}(s,a) \right\vert \right] \\
=& \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \upsilon_{t+1}^{-1}(s,a) f_{\theta_{n}^{t+1}}(s,a) - \upsilon_{t+1}^{-1}(s,a) f_{\theta^{t+1}}^{0}(s,a) \right\vert \right] + \mathcal{O} \left( \sup \left\vert \upsilon_{t+1}^{-1}(s,a) \right\vert R_{\theta}^{3/2} m^{-1/4} \right) \\
=& \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \upsilon_{t+1}^{-1}(s,a) f_{\theta_{n}^{t+1}}(s,a) - \sum_{i} q_{i} \upsilon_{t+1}^{-1}(s,a) f_{\theta^{t+1}_{i}}^{0}(s,a) \right\vert \right] + \mathcal{O} \left( \sup \left\vert \upsilon_{t+1}^{-1}(s,a) \right\vert R_{\theta}^{3/2} m^{-1/4} \right) \\
\le& \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \upsilon_{t+1}^{-1}(s,a) f_{\theta_{n}^{t+1}}(s,a) - \sum_{i} q_{i} \upsilon_{t+1}^{-1}(s,a) f_{\theta^{t+1}_{i}}(s,a) \right\vert \right. \nonumber \\
& \left. + \left\vert \sum_{i} q_{i} \upsilon_{t+1}^{-1}(s,a) f_{\theta^{t+1}_{i}}(s,a) - \sum_{i} q_{i} \upsilon_{t+1}^{-1}(s,a) f_{\theta^{t+1}_{i}}^{0}(s,a) \right\vert \right] + \mathcal{O} \left( \sup \left\vert \upsilon_{t+1}^{-1}(s,a) \right\vert R_{\theta}^{3/2} m^{-1/4} \right) \\
\le& \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \upsilon_{t+1}^{-1}(s,a) f_{\theta_{n}^{t+1}}(s,a) - \sum_{i} q_{i} \upsilon_{t+1}^{-1}(s,a) f_{\theta^{t+1}_{i}}(s,a) \right\vert \right] + 2 \mathcal{O} \left( \sup \left\vert \upsilon_{t+1}^{-1}(s,a) \right\vert R_{\theta}^{3/2} m^{-1/4} \right) \\
\le& \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \upsilon_{t+1}^{-1}(s,a) f_{\theta_{n}^{t+1}}(s,a) - \left( \beta_{t}^{-1} Q^{w^{t}}(s,a) + \upsilon_{t}^{-1}(s,a) f_{\theta^{t}}(s,a) \right) \right\vert \right. \nonumber \\
& \left. + \sum_{i} q_{i} \left\vert \left( \beta_{t}^{-1} Q^{w^{t}}(s,a) + \upsilon_{t}^{-1}(s,a) f_{\theta^{t}}(s,a) \right) - \left( \beta_{t}^{-1} Q^{w^{t}}(s,a) + \upsilon_{t}^{-1}(s,a) f_{\theta^{t}}(s,a) \right) \right\vert \right. \nonumber \\
& \left. + \sum_{i} q_{i} \left\vert \upsilon_{t+1}^{-1}(s,a) f_{\theta_{i}^{t+1}}(s,a) - \left( \beta_{t}^{-1} Q^{w^{t}}(s,a) + \upsilon_{t}^{-1}(s,a) f_{\theta^{t}}(s,a) \right) \right\vert \right] + 2 \mathcal{O} \left( \sup \left\vert \upsilon_{t+1}^{-1}(s,a) \right\vert R_{\theta}^{3/2} m^{-1/4} \right) \\
=& \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \upsilon_{t+1}^{-1}(s,a) f_{\theta_{n}^{t+1}}(s,a) - \left( \beta_{t}^{-1} Q^{w^{t}}(s,a) + \upsilon_{t}^{-1}(s,a) f_{\theta^{t}}(s,a) \right) \right\vert \right. \nonumber \\
& \left. + \beta_{t}^{-1} \sum_{i} q_{i} \left\vert Q^{w^{t}}(s,a) - Q^{w^{t}}(s,a) \right\vert \right. \nonumber \\
& \left. + \sum_{i} q_{i} \left\vert \upsilon_{t+1}^{-1}(s,a) f_{\theta_{i}^{t+1}}(s,a) - \left( \beta_{t}^{-1} Q^{w^{t}}(s,a) + \upsilon_{t}^{-1}(s,a) f_{\theta^{t}}(s,a) \right) \right\vert \right] + 2 \mathcal{O} \left( \sup \left\vert \upsilon_{t+1}^{-1}(s,a) \right\vert R_{\theta}^{3/2} m^{-1/4} \right) \\
\le& 2 \mathbb{E}_{n \thicksim C} \left[ \sup \left\vert \upsilon_{t+1}^{-1}(s,a) \right\vert \tilde{\epsilon}_{n}^{t+1} \xi^{t+1}_{n} \right] + 2 \mathcal{O} \left( \sup \left\vert \upsilon_{t+1}^{-1}(s,a) \right\vert R_{\theta}^{3/2} m^{-1/4} \right).
\end{alignat}
\end{lemma}
\end{proof}

\section{Proof of Lemma \ref{lemma:omega}\label{proof:lemma:omega}}

\begin{proof}
\begin{lemma}
For energy-based policy,
\begin{alignat}{1}
-\Omega_{CA} &= -\sum_{s} \sum_{n} q_{n} \rho_{\pi^{\ast},n}(s) \left< \log \left( \pi^{\theta^{t+1}}(\cdot \vert s) / \pi^{\theta^{t+1}_{n}}(\cdot \vert s) \right), \pi^{\ast} \right> \\
&= \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \log \pi^{\theta_{n}^{t+1}}(s,a) - \log \pi^{\theta^{t+1}}(s,a) \right] \\
&= \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \tau^{-1}_{t+1} f_{\theta_{n}^{t+1}}(s,a) - \tau^{-1}_{t+1} f_{\theta^{t+1}}(s,a) \right] \\
&\le \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \tau_{t+1}^{-1} f_{\theta_{n}^{t+1}}(s,a) - \tau_{t+1}^{-1} f_{\theta^{t+1}}(s,a) \right\vert \right] \\
&\le 2 \mathbb{E}_{n \thicksim C} \left[ \tau_{t+1}^{-1} \epsilon^{t+1}_{n} \xi^{t+1}_{n} \right] + \beta_{t}^{-1} \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \sum_{i} q_{i} \left\vert Q^{w^{t}_{n}}(s,a) - Q^{w^{t}_{i}}(s,a) \right\vert \right] + 2 \mathcal{O} \left( \tau_{t+1}^{-1} R_{\theta}^{3/2} m^{-1/4} \right).
\end{alignat}
For stochastic Gaussian policy,
\begin{alignat}{1}
-\Omega_{CA} &= -\sum_{s} \sum_{n} q_{n} \rho_{\pi^{\ast},n}(s) \left< \log \left( \pi^{\theta^{t+1}}(\cdot \vert s) / \pi^{\theta^{t+1}_{n}}(\cdot \vert s) \right), \pi^{\ast} \right> \\
&= \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \log \pi^{\theta_{n}^{t+1}} - \log \pi^{\theta^{t+1}} \right] \\
&= \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ - \frac{\left( a - f_{\theta^{t+1}_{n}}(s,a) \right)^2}{2 \sigma_{t+1}^{2}} - \log \sqrt{2 \pi} \sigma_{t+1} + \frac{\left( a - f_{\theta^{t+1}}(s,a) \right)^2}{2 \sigma_{t+1}^{2}} + \log \sqrt{2 \pi} \sigma_{t+1} \right] \\
&= \frac{1}{2 \sigma_{t+1}^{2}} \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left( a - f_{\theta^{t+1}}(s,a) \right)^2 - \left( a - f_{\theta^{t+1}_{n}}(s,a) \right)^2 \right] \\
&= \frac{1}{2 \sigma_{t+1}^{2}} \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left( a - f_{\theta^{0}}(s,a) \right)^2 + 2 \left( f_{\theta^{0}}(s,a) - a \right) \left( f_{\theta^{t+1}}(s,a) - f_{\theta^{0}}(s,a) \right) \right. \\
& \quad + 2 \left( f_{\theta^{t+1}}(s,a) - f_{\theta^{0}}(s,a) \right)^{2} - \left( a - f_{\theta^{0}}(s,a) \right)^2 - 2 \left( f_{\theta^{0}}(s,a) - a \right) \left( f_{\theta^{t+1}_{n}}(s,a) - f_{\theta^{0}}(s,a) \right) \\
& \quad \left. - 2 \left( f_{\theta^{t+1}_{n}}(s,a) - f_{\theta^{0}}(s,a) \right)^2 \right] \\
&= \frac{1}{2 \sigma_{t+1}^{2}} \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ 2 \left( f_{\theta^{0}}(s,a) - a \right) \left( f_{\theta^{t+1}}(s,a) - f_{\theta^{t+1}_{n}}(s,a) \right) \right. \\
& \quad \left. + 2 \left( f_{\theta^{t+1}}(s,a) - f_{\theta^{0}}(s,a) \right)^{2} - 2 \left( f_{\theta^{t+1}_{n}}(s,a) - f_{\theta^{0}}(s,a) \right)^2 \right] \\
&\le \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \frac{f_{\theta^{0}}(s,a) - a}{\sigma_{t+1}^{2}} \left( f_{\theta^{t+1}}(s,a) - f_{\theta^{t+1}_{n}}(s,a) \right) \right] + \frac{R_{\theta}^{2}}{\sigma_{t+1}^{2}} \\
&\le \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \upsilon_{t+1}^{-1}(s,a) f_{\theta^{t+1}}(s,a) - \upsilon_{t+1}^{-1}(s,a) f_{\theta^{t+1}_{n}}(s,a) \right\vert \right] + \frac{R_{\theta}^{2}}{\sigma_{t+1}^{2}} \\
\le& 2 \mathbb{E}_{n \thicksim C} \left[ \sup \left\vert \upsilon_{t+1}^{-1}(s,a) \right\vert \tilde{\epsilon}_{n}^{t+1} \xi^{t+1}_{n} \right] + \beta_{t}^{-1} \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \sum_{i} q_{i} \left\vert Q^{w^{t}_{n}}(s,a) - Q^{w^{t}_{i}}(s,a) \right\vert \right] \nonumber \\
& + 2 \mathcal{O} \left( \sup \left\vert \upsilon_{t+1}^{-1}(s,a) \right\vert R_{\theta}^{3/2} m^{-1/4} \right) + \frac{R_{\theta}^{2}}{\sigma_{t+1}^{2}}.
\end{alignat}
\end{lemma}


\begin{lemma}
For energy-based policy,
\begin{alignat}{1}
-\Omega_{AC} &= -\sum_{s} \sum_{n} q_{n} \rho_{\pi^{\ast},n}(s) \left< \log \left( \pi^{\theta^{t+1}}(\cdot \vert s) / \pi^{\theta^{t+1}_{n}}(\cdot \vert s) \right), \pi^{\ast} \right> \\
&= \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \log \pi^{\theta_{n}^{t+1}}(s,a) - \log \pi^{\theta^{t+1}}(s,a) \right] \\
&= \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \tau^{-1}_{t+1} f_{\theta_{n}^{t+1}}(s,a) - \tau^{-1}_{t+1} f_{\theta^{t+1}}(s,a) \right] \\
&\le \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \tau_{t+1}^{-1} f_{\theta_{n}^{t+1}}(s,a) - \tau_{t+1}^{-1} f_{\theta^{t+1}}(s,a) \right\vert \right] \\
&\le 2 \mathbb{E}_{n \thicksim C} \left[ \tau_{t+1}^{-1} \epsilon^{t+1}_{n} \xi^{t+1}_{n} \right] + 2 \tau_{t+1}^{-1} \mathcal{O} \left( R_{\theta}^{3/2} m^{-1/4} \right).
\end{alignat}
For stochastic Gaussian policy,
\begin{alignat}{1}
-\Omega_{AC} &= -\sum_{s} \sum_{n} q_{n} \rho_{\pi^{\ast},n}(s) \left< \log \left( \pi^{\theta^{t+1}}(\cdot \vert s) / \pi^{\theta^{t+1}_{n}}(\cdot \vert s) \right), \pi^{\ast} \right> \\
&= \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \log \pi^{\theta_{n}^{t+1}} - \log \pi^{\theta^{t+1}} \right] \\
&= \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ - \frac{\left( a - f_{\theta^{t+1}_{n}}(s,a) \right)^2}{2 \sigma_{t+1}^{2}} - \log \sqrt{2 \pi} \sigma_{t+1} + \frac{\left( a - f_{\theta^{t+1}}(s,a) \right)^2}{2 \sigma_{t+1}^{2}} + \log \sqrt{2 \pi} \sigma_{t+1} \right] \\
&= \frac{1}{2 \sigma_{t+1}^{2}} \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left( a - f_{\theta^{t+1}}(s,a) \right)^2 - \left( a - f_{\theta^{t+1}_{n}}(s,a) \right)^2 \right] \\
&= \frac{1}{2 \sigma_{t+1}^{2}} \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left( a - f_{\theta^{0}}(s,a) \right)^2 + 2 \left( f_{\theta^{0}}(s,a) - a \right) \left( f_{\theta^{t+1}}(s,a) - f_{\theta^{0}}(s,a) \right) \right. \\
& \quad + 2 \left( f_{\theta^{t+1}}(s,a) - f_{\theta^{0}}(s,a) \right)^{2} - \left( a - f_{\theta^{0}}(s,a) \right)^2 - 2 \left( f_{\theta^{0}}(s,a) - a \right) \left( f_{\theta^{t+1}_{n}}(s,a) - f_{\theta^{0}}(s,a) \right) \\
& \quad \left. - 2 \left( f_{\theta^{t+1}_{n}}(s,a) - f_{\theta^{0}}(s,a) \right)^2 \right] \\
&= \frac{1}{2 \sigma_{t+1}^{2}} \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ 2 \left( f_{\theta^{0}}(s,a) - a \right) \left( f_{\theta^{t+1}}(s,a) - f_{\theta^{t+1}_{n}}(s,a) \right) \right. \\
& \quad \left. + 2 \left( f_{\theta^{t+1}}(s,a) - f_{\theta^{0}}(s,a) \right)^{2} - 2 \left( f_{\theta^{t+1}_{n}}(s,a) - f_{\theta^{0}}(s,a) \right)^2 \right] \\
&\le \frac{1}{\sigma_{t+1}^{2}} \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left( f_{\theta^{0}}(s,a) - a \right) \left( f_{\theta^{t+1}}(s,a) - f_{\theta^{t+1}_{n}}(s,a) \right) \right] + \frac{R_{\theta}^{2}}{\sigma_{t+1}^{2}} \\
&\le \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \left( \upsilon^{-1}_{t+1}(s,a) f_{\theta^{t+1}}(s,a) - \upsilon^{-1}_{t+1}(s,a) f_{\theta^{t+1}_{n}}(s,a) \right\vert \right) \right] + \frac{R_{\theta}^{2}}{\sigma_{t+1}^{2}} \\
\le& 2 \mathbb{E}_{n \thicksim C} \left[ \sup \left\vert \upsilon_{t+1}^{-1}(s,a) \right\vert \tilde{\epsilon}_{n}^{t+1} \xi^{t+1}_{n} \right] + 2 \mathcal{O} \left( \sup \left\vert \upsilon_{t+1}^{-1}(s,a) \right\vert R_{\theta}^{3/2} m^{-1/4} \right) + \frac{R_{\theta}^{2}}{\sigma_{t+1}^{2}}.
\end{alignat}
\end{lemma}
\end{proof}

\section{Proof of Lemma \ref{lemma:omega}\label{proof:lemma:omega}}

\begin{proof}
For energy-based policy,
\begin{alignat}{1}
-\Omega_{CA} &= -\sum_{s} \sum_{n} q_{n} \rho_{\pi^{\ast},n}(s) \left< \log \left( \pi^{\theta^{t+1}}(\cdot \vert s) / \pi^{\theta^{t+1}_{n}}(\cdot \vert s) \right), \pi^{\ast} \right> \\
&= \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \log \pi^{\theta_{n}^{t+1}}(s,a) - \log \pi^{\theta^{t+1}}(s,a) \right] \\
&= \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \tau^{-1}_{t+1} f_{\theta_{n}^{t+1}}(s,a) - \tau^{-1}_{t+1} f_{\theta^{t+1}}(s,a) \right] \\
&\le \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \tau_{t+1}^{-1} f_{\theta_{n}^{t+1}}(s,a) - \tau_{t+1}^{-1} f_{\theta^{t+1}}(s,a) \right\vert \right] \\
&\le 2 \mathbb{E}_{n \thicksim C} \left[ \tau_{t+1}^{-1} \epsilon^{t+1}_{n} \xi^{t+1}_{n} \right] + \beta_{t}^{-1} \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \sum_{i} q_{i} \left\vert Q^{w^{t}_{n}}(s,a) - Q^{w^{t}_{i}}(s,a) \right\vert \right] + 2 \mathcal{O} \left( \tau_{t+1}^{-1} R_{\theta}^{3/2} m^{-1/4} \right).
\end{alignat}
For stochastic Gaussian policy,
\begin{alignat}{1}
-\Omega_{CA} &= -\sum_{s} \sum_{n} q_{n} \rho_{\pi^{\ast},n}(s) \left< \log \left( \pi^{\theta^{t+1}}(\cdot \vert s) / \pi^{\theta^{t+1}_{n}}(\cdot \vert s) \right), \pi^{\ast} \right> \\
&= \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \log \pi^{\theta_{n}^{t+1}} - \log \pi^{\theta^{t+1}} \right] \\
&= \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ - \frac{\left( a - f_{\theta^{t+1}_{n}}(s,a) \right)^2}{2 \sigma_{t+1}^{2}} - \log \sqrt{2 \pi} \sigma_{t+1} + \frac{\left( a - f_{\theta^{t+1}}(s,a) \right)^2}{2 \sigma_{t+1}^{2}} + \log \sqrt{2 \pi} \sigma_{t+1} \right] \\
&= \frac{1}{2 \sigma_{t+1}^{2}} \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left( a - f_{\theta^{t+1}}(s,a) \right)^2 - \left( a - f_{\theta^{t+1}_{n}}(s,a) \right)^2 \right] \\
&= \frac{1}{2 \sigma_{t+1}^{2}} \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left( a - f_{\theta^{0}}(s,a) \right)^2 + 2 \left( f_{\theta^{0}}(s,a) - a \right) \left( f_{\theta^{t+1}}(s,a) - f_{\theta^{0}}(s,a) \right) \right. \\
& \quad + 2 \left( f_{\theta^{t+1}}(s,a) - f_{\theta^{0}}(s,a) \right)^{2} - \left( a - f_{\theta^{0}}(s,a) \right)^2 - 2 \left( f_{\theta^{0}}(s,a) - a \right) \left( f_{\theta^{t+1}_{n}}(s,a) - f_{\theta^{0}}(s,a) \right) \\
& \quad \left. - 2 \left( f_{\theta^{t+1}_{n}}(s,a) - f_{\theta^{0}}(s,a) \right)^2 \right] \\
&= \frac{1}{2 \sigma_{t+1}^{2}} \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ 2 \left( f_{\theta^{0}}(s,a) - a \right) \left( f_{\theta^{t+1}}(s,a) - f_{\theta^{t+1}_{n}}(s,a) \right) \right. \\
& \quad \left. + 2 \left( f_{\theta^{t+1}}(s,a) - f_{\theta^{0}}(s,a) \right)^{2} - 2 \left( f_{\theta^{t+1}_{n}}(s,a) - f_{\theta^{0}}(s,a) \right)^2 \right] \\
&\le \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \frac{f_{\theta^{0}}(s,a) - a}{\sigma_{t+1}^{2}} \left( f_{\theta^{t+1}}(s,a) - f_{\theta^{t+1}_{n}}(s,a) \right) \right] + \frac{R_{\theta}^{2}}{\sigma_{t+1}^{2}} \\
&\le \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \upsilon_{t+1}^{-1}(s,a) f_{\theta^{t+1}}(s,a) - \upsilon_{t+1}^{-1}(s,a) f_{\theta^{t+1}_{n}}(s,a) \right\vert \right] + \frac{R_{\theta}^{2}}{\sigma_{t+1}^{2}} \\
\le& 2 \mathbb{E}_{n \thicksim C} \left[ \sup \left\vert \upsilon_{t+1}^{-1}(s,a) \right\vert \tilde{\epsilon}_{n}^{t+1} \xi^{t+1}_{n} \right] + \beta_{t}^{-1} \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \sum_{i} q_{i} \left\vert Q^{w^{t}_{n}}(s,a) - Q^{w^{t}_{i}}(s,a) \right\vert \right] \nonumber \\
& + 2 \mathcal{O} \left( \sup \left\vert \upsilon_{t+1}^{-1}(s,a) \right\vert R_{\theta}^{3/2} m^{-1/4} \right) + \frac{R_{\theta}^{2}}{\sigma_{t+1}^{2}}.
\end{alignat}

For energy-based policy,
\begin{alignat}{1}
-\Omega_{AC} &= -\sum_{s} \sum_{n} q_{n} \rho_{\pi^{\ast},n}(s) \left< \log \left( \pi^{\theta^{t+1}}(\cdot \vert s) / \pi^{\theta^{t+1}_{n}}(\cdot \vert s) \right), \pi^{\ast} \right> \\
&= \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \log \pi^{\theta_{n}^{t+1}}(s,a) - \log \pi^{\theta^{t+1}}(s,a) \right] \\
&= \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \tau^{-1}_{t+1} f_{\theta_{n}^{t+1}}(s,a) - \tau^{-1}_{t+1} f_{\theta^{t+1}}(s,a) \right] \\
&\le \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \tau_{t+1}^{-1} f_{\theta_{n}^{t+1}}(s,a) - \tau_{t+1}^{-1} f_{\theta^{t+1}}(s,a) \right\vert \right] \\
&\le 2 \mathbb{E}_{n \thicksim C} \left[ \tau_{t+1}^{-1} \epsilon^{t+1}_{n} \xi^{t+1}_{n} \right] + 2 \tau_{t+1}^{-1} \mathcal{O} \left( R_{\theta}^{3/2} m^{-1/4} \right).
\end{alignat}
For stochastic Gaussian policy,
\begin{alignat}{1}
-\Omega_{AC} &= -\sum_{s} \sum_{n} q_{n} \rho_{\pi^{\ast},n}(s) \left< \log \left( \pi^{\theta^{t+1}}(\cdot \vert s) / \pi^{\theta^{t+1}_{n}}(\cdot \vert s) \right), \pi^{\ast} \right> \\
&= \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \log \pi^{\theta_{n}^{t+1}} - \log \pi^{\theta^{t+1}} \right] \\
&= \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ - \frac{\left( a - f_{\theta^{t+1}_{n}}(s,a) \right)^2}{2 \sigma_{t+1}^{2}} - \log \sqrt{2 \pi} \sigma_{t+1} + \frac{\left( a - f_{\theta^{t+1}}(s,a) \right)^2}{2 \sigma_{t+1}^{2}} + \log \sqrt{2 \pi} \sigma_{t+1} \right] \\
&= \frac{1}{2 \sigma_{t+1}^{2}} \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left( a - f_{\theta^{t+1}}(s,a) \right)^2 - \left( a - f_{\theta^{t+1}_{n}}(s,a) \right)^2 \right] \\
&= \frac{1}{2 \sigma_{t+1}^{2}} \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left( a - f_{\theta^{0}}(s,a) \right)^2 + 2 \left( f_{\theta^{0}}(s,a) - a \right) \left( f_{\theta^{t+1}}(s,a) - f_{\theta^{0}}(s,a) \right) \right. \\
& \quad + 2 \left( f_{\theta^{t+1}}(s,a) - f_{\theta^{0}}(s,a) \right)^{2} - \left( a - f_{\theta^{0}}(s,a) \right)^2 - 2 \left( f_{\theta^{0}}(s,a) - a \right) \left( f_{\theta^{t+1}_{n}}(s,a) - f_{\theta^{0}}(s,a) \right) \\
& \quad \left. - 2 \left( f_{\theta^{t+1}_{n}}(s,a) - f_{\theta^{0}}(s,a) \right)^2 \right] \\
&= \frac{1}{2 \sigma_{t+1}^{2}} \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ 2 \left( f_{\theta^{0}}(s,a) - a \right) \left( f_{\theta^{t+1}}(s,a) - f_{\theta^{t+1}_{n}}(s,a) \right) \right. \\
& \quad \left. + 2 \left( f_{\theta^{t+1}}(s,a) - f_{\theta^{0}}(s,a) \right)^{2} - 2 \left( f_{\theta^{t+1}_{n}}(s,a) - f_{\theta^{0}}(s,a) \right)^2 \right] \\
&\le \frac{1}{\sigma_{t+1}^{2}} \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left( f_{\theta^{0}}(s,a) - a \right) \left( f_{\theta^{t+1}}(s,a) - f_{\theta^{t+1}_{n}}(s,a) \right) \right] + \frac{R_{\theta}^{2}}{\sigma_{t+1}^{2}} \\
&\le \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \left( \upsilon^{-1}_{t+1}(s,a) f_{\theta^{t+1}}(s,a) - \upsilon^{-1}_{t+1}(s,a) f_{\theta^{t+1}_{n}}(s,a) \right\vert \right) \right] + \frac{R_{\theta}^{2}}{\sigma_{t+1}^{2}} \\
\le& 2 \mathbb{E}_{n \thicksim C} \left[ \sup \left\vert \upsilon_{t+1}^{-1}(s,a) \right\vert \tilde{\epsilon}_{n}^{t+1} \xi^{t+1}_{n} \right] + 2 \mathcal{O} \left( \sup \left\vert \upsilon_{t+1}^{-1}(s,a) \right\vert R_{\theta}^{3/2} m^{-1/4} \right) + \frac{R_{\theta}^{2}}{\sigma_{t+1}^{2}}.
\end{alignat}
\end{proof}

\section{Proof of Theorem \ref{theorem:global_convergence_rate}\label{proof:theorem:global_convergence_rate}}

\begin{proof}
For the baseline with action-value function $Q^{w^{t}_{n}}$, we have
\begin{alignat}{1}
& D_{KL}(\pi^{\ast}(\cdot \vert s) \Vert \pi^{\theta^{t}}(\cdot \vert s)) - D_{KL}(\pi^{\ast}(\cdot \vert s) \Vert \pi^{\theta^{t+1}}(\cdot \vert s)) \\
=& D_{KL}(\pi^{\ast}(\cdot \vert s) \Vert \pi^{\theta^{t}}(\cdot \vert s)) - D_{KL}(\pi^{\ast}(\cdot \vert s) \Vert \pi^{\theta^{t+1}_{n}}(\cdot \vert s)) + D_{KL}(\pi^{\ast}(\cdot \vert s) \Vert \pi^{\theta^{t+1}_{n}}(\cdot \vert s)) - D_{KL}(\pi^{\ast}(\cdot \vert s) \Vert \pi^{\theta^{t+1}}(\cdot \vert s)) \\
=& \left< \log \left( \pi^{\theta^{t+1}_{n}}(\cdot \vert s) / \pi^{\theta^{t}}(\cdot \vert s) \right) - \beta_{t}^{-1} Q_{n}^{\pi^{\theta^{t}}}(s,\cdot), \pi^{\ast}(\cdot \vert s) - \pi^{\theta^{t}}(\cdot \vert s) \right> + \beta_{t}^{-1} \left< Q_{n}^{\pi^{\theta^{t}}}(s,\cdot), \pi^{\ast}(\cdot \vert s) - \pi^{\theta^{t}}(\cdot \vert s) \right> \\
& + D_{KL}(\pi^{\theta_{n}^{t+1}}(\cdot \vert s) \Vert \pi^{\theta^{t}}(\cdot \vert s)) + \left< \log \left( \pi^{\theta^{t+1}_{n}}(\cdot \vert s) / \pi^{\theta^{t}}(\cdot \vert s) \right), \pi^{\theta_{t}}(\cdot \vert s) - \pi^{\theta^{t+1}_{n}}(\cdot \vert s) \right> \\
& + \left< \log \left( \pi^{\theta^{t+1}}(\cdot \vert s) / \pi^{\theta^{t+1}_{n}}(\cdot \vert s) \right), \pi^{\ast}(\cdot \vert s) \right>.
\end{alignat}
By taking expectation with respect to $n \thicksim C$ and $s \thicksim \rho_{\pi^{\ast},n}$, we have
\begin{alignat}{1}
& \sum_{s} \sum_{n} q_{n} \rho_{\pi^{\ast},n}(s) \left( D_{KL}(\pi^{\ast}(\cdot \vert s) \Vert \pi^{\theta^{t+1}}(\cdot \vert s)) - D_{KL}(\pi^{\ast}(\cdot \vert s) \Vert \pi^{\theta^{t}}(\cdot \vert s)) \right) \\
=& \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}} \left[ D_{KL}(\pi^{\ast}(\cdot \vert s) \Vert \pi^{\theta^{t+1}}(\cdot \vert s)) - D_{KL}(\pi^{\ast}(\cdot \vert s) \Vert \pi^{\theta^{t}}(\cdot \vert s)) \right] \\
=& \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}} \left[ - \left< \log \left( \pi^{\theta^{t+1}_{n}}(\cdot \vert s) / \pi^{\theta^{t}}(\cdot \vert s) \right) - \beta_{t}^{-1} Q_{n}^{\pi^{\theta^{t}}}(s,\cdot), \pi^{\ast}(\cdot \vert s) - \pi^{\theta^{t}}(\cdot \vert s) \right> \right. \\
& - \beta_{t}^{-1} \left< Q_{n}^{\pi^{\theta^{t}}}(s,\cdot), \pi^{\ast}(\cdot \vert s) - \pi^{\theta^{t}}(\cdot \vert s) \right> - \left< \log \left( \pi^{\theta^{t+1}}(\cdot \vert s) / \pi^{\theta^{t+1}_{n}}(\cdot \vert s) \right), \pi^{\ast}(\cdot \vert s) \right> \\
& \left. - D_{KL}(\pi^{\theta_{n}^{t+1}}(\cdot \vert s) \Vert \pi^{\theta^{t}}(\cdot \vert s)) - \left< \log \left( \pi^{\theta^{t+1}_{n}}(\cdot \vert s) / \pi^{\theta^{t}}(\cdot \vert s) \right), \pi^{\theta_{t}}(\cdot \vert s) - \pi^{\theta^{t+1}_{n}}(\cdot \vert s) \right> \right].
\end{alignat}

For FedRAC with action-value function $Q^{w^{t}}$, we have
\begin{alignat}{1}
& D_{KL}(\pi^{\ast}(\cdot \vert s) \Vert \pi^{\theta^{t}}(\cdot \vert s)) - D_{KL}(\pi^{\ast}(\cdot \vert s) \Vert \pi^{\theta^{t+1}}(\cdot \vert s)) \\
=& D_{KL}(\pi^{\ast}(\cdot \vert s) \Vert \pi^{\theta^{t}}(\cdot \vert s)) - D_{KL}(\pi^{\ast}(\cdot \vert s) \Vert \pi^{\theta^{t+1}_{n}}(\cdot \vert s)) + D_{KL}(\pi^{\ast}(\cdot \vert s) \Vert \pi^{\theta^{t+1}_{n}}(\cdot \vert s)) - D_{KL}(\pi^{\ast}(\cdot \vert s) \Vert \pi^{\theta^{t+1}}(\cdot \vert s)) \\
=& \left< \log \left( \pi^{\theta^{t+1}_{n}}(\cdot \vert s) / \pi^{\theta^{t}}(\cdot \vert s) \right) - \beta_{t}^{-1} \sum_{i} \frac{q_{i} \rho_{\pi^{\ast},i}(s)}{Z_{\pi^{\ast}}(s)} Q_{i}^{\pi^{\theta^{t}}}(s,\cdot), \pi^{\ast}(\cdot \vert s) - \pi^{\theta^{t}}(\cdot \vert s) \right> \\
& + \beta_{t}^{-1} \left< \sum_{i} \frac{q_{i} \rho_{i}(s)}{Z_{\pi^{\ast}}(s)} Q_{i}^{\pi^{\theta^{t}}}(s,\cdot), \pi^{\ast}(\cdot \vert s) - \pi^{\theta^{t}}(\cdot \vert s) \right> + \left< \log \left( \pi^{\theta^{t+1}}(\cdot \vert s) / \pi^{\theta^{t+1}_{n}}(\cdot \vert s) \right), \pi^{\ast}(\cdot \vert s) \right> \\
& + D_{KL}(\pi^{\theta_{n}^{t+1}}(\cdot \vert s) \Vert \pi^{\theta^{t}}(\cdot \vert s)) + \left< \log \left( \pi^{\theta^{t+1}_{n}}(\cdot \vert s) / \pi^{\theta^{t}}(\cdot \vert s) \right), \pi^{\theta_{t}}(\cdot \vert s) - \pi^{\theta^{t+1}_{n}}(\cdot \vert s) \right>.
\end{alignat}


\begin{alignat}{1}
& \sum_{s} \sum_{n} q_{n} \rho_{\pi^{\ast},n}(s) \left( D_{KL}(\pi^{\ast}(\cdot \vert s) \Vert \pi^{\theta^{t+1}}(\cdot \vert s)) - D_{KL}(\pi^{\ast}(\cdot \vert s) \Vert \pi^{\theta^{t}}(\cdot \vert s)) \right) \\
=& \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}} \left[ D_{KL}(\pi^{\ast}(\cdot \vert s) \Vert \pi^{\theta^{t+1}}(\cdot \vert s)) - D_{KL}(\pi^{\ast}(\cdot \vert s) \Vert \pi^{\theta^{t}}(\cdot \vert s)) \right] \\
=& \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}} \left[ - \left< \log \left( \pi^{\theta^{t+1}_{n}}(\cdot \vert s) / \pi^{\theta^{t}}(\cdot \vert s) \right) - \beta_{t}^{-1} \sum_{n} \frac{q_{i} \rho_{\pi^{\ast},i}(s)}{Z_{\pi^{\ast}}(s)} Q_{i}^{\pi^{\theta^{t}}}(s,\cdot), \pi^{\ast}(\cdot \vert s) - \pi^{\theta^{t}}(\cdot \vert s) \right> \right. \\
& - \beta_{t}^{-1} \left< \sum_{i} \frac{q_{i} \rho_{\pi^{\ast},i}(s)}{Z_{\pi^{\ast}}(s)} Q_{i}^{\pi^{\theta^{t}}}(s,\cdot), \pi^{\ast}(\cdot \vert s) - \pi^{\theta^{t}}(\cdot \vert s) \right> \\
& - D_{KL}(\pi^{\theta_{n}^{t+1}}(\cdot \vert s) \Vert \pi^{\theta^{t}}(\cdot \vert s)) - \left< \log \left( \pi^{\theta^{t+1}_{n}}(\cdot \vert s) / \pi^{\theta^{t}}(\cdot \vert s) \right), \pi^{\theta_{t}}(\cdot \vert s) - \pi^{\theta^{t+1}_{n}}(\cdot \vert s) \right> \\
& \left. - \left< \log \left( \pi^{\theta^{t+1}}(\cdot \vert s) / \pi^{\theta^{t+1}_{n}}(\cdot \vert s) \right), \pi^{\ast}(\cdot \vert s) \right> \right].
\end{alignat}

\begin{alignat}{1}
\min_{0 \le t \le T} \eta(\pi^{\ast}) - \eta(\pi^{\theta^{t}}) \le \frac{\log \vert \mathcal{A} \vert + M \sum_{t=0}^{T}\beta_{t}^{-2} + \sum_{t=1}^{T}(\varepsilon^{t} + \dot{\varepsilon}^{t}) + \Omega_{CA}}{\sum_{t=1}^{T}\beta_{t}^{-1}}
\end{alignat}
\end{proof}

\section{Proof of Lemma \ref{lemma:omega}\label{proof:lemma:omega}}

We need the following lemma for proving Lemma \ref{lemma:omega}.
\begin{lemma}
\label{lemma:changing_action_error}
Given parameter $\theta$ and any pair of action $a$ and $a^{\prime}$, we have
\begin{alignat}{1}
\mathbb{E}_{\text{init}} \left\vert \left[ u_{\vartheta}(s,a) - u_{\vartheta}(s,a^{\prime}) \right\vert \right] &\le 2 R_{\vartheta}^{2} + \mathcal{O} \left( 1 \right), \\
\mathbb{E}_{\text{init}} \left\vert \left[ u_{\vartheta}(s,a) - u_{\vartheta^{\prime}}(s,a^{\prime}) \right\vert \right] &\le 20 R_{\vartheta}^{2} + \mathcal{O} \left( 1 \right).
\end{alignat}
\end{lemma}
\begin{proof}
By the Jensen's inequality and the Cauchy-Schwarz inequality, we have
\begin{alignat}{1}
\mathbb{E}_{\text{init}} \left\vert \left[ u_{\vartheta}(s,a) - u_{\vartheta}(s,a^{\prime}) \right\vert \right]^{2} &\le \mathbb{E}_{\text{init}} \left\vert \left[ u_{\vartheta}(s,a) - u_{\vartheta}(s,a^{\prime}) \right\vert^{2} \right] \nonumber \\
&= \mathbb{E}_{\text{init}} \left[ \left\vert \frac{1}{\sqrt{m}} \sum_{i}^{m} b_{i} \cdot \mathbf{1} \left\{ [\vartheta]_{i}^{T}(s,a) > 0 \right\} [\vartheta]_{i}^{T} (s,a - a^{\prime}) \right\vert^{2} \right] \\
&\le \frac{1}{m} \mathbb{E}_{\text{init}} \left[ \left( \sum_{i}^{m} \left( b_{i} \cdot \mathbf{1} \left\{ [\vartheta]_{i}^{T}(s,a) > 0 \right\} \right)^{2} \right) \cdot \left( \sum_{i}^{m} \left( [\vartheta]_{i}^{T} (s,a - a^{\prime}) \right)^{2} \right) \right] \\
\end{alignat}
Furthermore, we have
\begin{alignat}{1}
\left\Vert \vartheta \right\Vert_{2}^{2} &\le \left( \left\Vert \vartheta - \vartheta^{0} \right\Vert_{2} + \left\Vert \vartheta^{0} \right\Vert_{2} \right)^{2} \le 2 R_{\vartheta}^{2} + 2 \left\Vert \vartheta^{0} \right\Vert_{2}^{2}. \label{eq:bound_vartheta}
\end{alignat}
Therefore, we can obtain
\begin{alignat}{1}
\mathbb{E}_{\text{init}} \left\vert \left[ u_{\vartheta}(s,a) - u_{\vartheta}(s,a^{\prime}) \right\vert \right]^{2} &\le \mathbb{E}_{\text{init}} \left[ \left\Vert \vartheta \right\Vert_{2}^{2} \right] \le 2 R_{\vartheta}^{2} + \mathcal{O} \left( 1 \right).
\end{alignat}
This completes the proof of the first part. Similarly, by the Jensen's inequality, we have
\begin{alignat}{1}
& \mathbb{E}_{\text{init}} \left\vert \left[ u_{\vartheta}(s,a) - u_{\vartheta^{\prime}}(s,a^{\prime}) \right\vert \right]^{2} \nonumber \\
&\le \frac{1}{m} \mathbb{E}_{\text{init}} \left[ \left\vert \sum_{i}^{m} b_{i} \cdot \mathbf{1} \left\{ [\vartheta]_{i}^{T}(s,a) > 0 \right\} [\vartheta]_{i}^{T} (s,a) - \sum_{i}^{m} b_{i} \cdot \mathbf{1} \left\{ [\vartheta^{\prime}]_{i}^{T}(s,a^{\prime}) > 0 \right\} [\vartheta^{\prime}]_{i}^{T} (s,a^{\prime}) \right\vert^{2} \right].
\end{alignat}
By the fact that $(a + b)^{2} \le 2a^{2} + 2b^{2}$ and $ab - cd = a(b-d) + d(a-c)$, we have
\begin{alignat}{1}
\mathbb{E}_{\text{init}} \left\vert \left[ u_{\vartheta}(s,a) - u_{\vartheta^{\prime}}(s,a^{\prime}) \right\vert \right]^{2} &\le \frac{1}{m} \mathbb{E}_{\text{init}} \left[ \left\vert \sum_{i}^{m} b_{i} \cdot \mathbf{1} \left\{ [\vartheta]_{i}^{T}(s,a) > 0 \right\} \left( [\vartheta]_{i}^{T} (s,a) - [\vartheta^{\prime}]_{i}^{T} (s,a^{\prime}) \right) \right. \right. \nonumber \\
& \left. \left. \quad + \sum_{i}^{m} b_{i} \cdot \left( \mathbf{1} \left\{ [\vartheta^{\prime}]_{i}^{T}(s,a^{\prime}) > 0 \right\} - \mathbf{1} \left\{ [\vartheta^{\prime}]_{i}^{T}(s,a^{\prime}) > 0 \right\} \right) [\vartheta^{\prime}]_{i}^{T} (s,a^{\prime}) \right\vert^{2} \right] \\
&\le \frac{1}{m} \mathbb{E}_{\text{init}} \left[ 2 \left\vert \sum_{i}^{m} b_{i} \cdot \mathbf{1} \left\{ [\vartheta]_{i}^{T}(s,a) > 0 \right\} \left( [\vartheta]_{i}^{T} (s,a) - [\vartheta^{\prime}]_{i}^{T} (s,a^{\prime}) \right) \right\vert^{2} \right. \nonumber \\
& \left. \quad + 2 \left\vert \sum_{i}^{m} b_{i} \cdot \left( \mathbf{1} \left\{ [\vartheta^{\prime}]_{i}^{T}(s,a^{\prime}) > 0 \right\} - \mathbf{1} \left\{ [\vartheta^{\prime}]_{i}^{T}(s,a^{\prime}) > 0 \right\} \right) [\vartheta^{\prime}]_{i}^{T} (s,a^{\prime}) \right\vert^{2} \right].
\end{alignat}
By (\ref{eq:bound_vartheta}) and the Cauchy-Schwarz inequality, we have
\begin{alignat}{1}
\mathbb{E}_{\text{init}} \left\vert \left[ u_{\vartheta}(s,a) - u_{\vartheta^{\prime}}(s,a^{\prime}) \right\vert \right]^{2} &\le 2 \mathbb{E}_{\text{init}} \left[ \left( \sum_{i}^{m} \left( [\vartheta]_{i}^{T} (s,a) - [\vartheta^{\prime}]_{i}^{T} (s,a^{\prime}) \right)^{2} \right) + \left\Vert \vartheta \right\Vert_{2}^{2} \right] \\
&\le 2 \mathbb{E}_{\text{init}} \left[ \left( \sum_{i}^{m} 2 \left( [\vartheta]_{i}^{T} (s,a) \right)^{2} + 2 \left( [\vartheta^{\prime}]_{i}^{T} (s,a^{\prime}) \right)^{2} \right) + \left\Vert \vartheta \right\Vert_{2}^{2} \right] \\
&\le 10 \mathbb{E}_{\text{init}} \left[ \left\Vert \vartheta \right\Vert_{2}^{2} \right] \\
&\le 20 R_{\vartheta}^{2} + \mathcal{O} \left( 1 \right).
\end{alignat}
\end{proof}

\begin{proof}
For Softmax policy, we have
\begin{alignat}{1}
\Omega^{t+1} &= \sum_{s} \sum_{n} q_{n} \rho_{\pi^{\ast},n}(s) \left< \log \left( \pi^{\theta^{t+1}}(\cdot \vert s) / \pi^{\theta^{t+1}_{n}}(\cdot \vert s) \right), \pi^{\ast} \right> \nonumber \\
&= \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \log \pi^{\theta^{t+1}}(s,a) - \log \pi^{\theta_{n}^{t+1}}(s,a) \right] \\
&= \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \tau^{-1}_{t+1} f_{\theta^{t+1}}(s,a) - \tau^{-1}_{t+1} f_{\theta_{n}^{t+1}}(s,a) + \log \sum_{a^{\prime}} \exp \left( \tau^{-1}_{t+1} f_{\theta_{n}^{t+1}}(s,a^{\prime}) \right) \right. \nonumber \\
& \left. \quad - \log \sum_{a^{\prime}} \exp \left( \tau^{-1}_{t+1} f_{\theta^{t+1}}(s,a^{\prime}) \right) \right]. \label{eq:proof:lemma:omega0}
\end{alignat}
The last two log-sum-exp terms on the RHS of (\ref{eq:proof:lemma:omega0}) can be bounded as follows. By the log-sum inequality, we can obtain
\begin{alignat}{1}
\log \sum_{a^{\prime}} \exp \left( \tau^{-1}_{t+1} f_{\theta_{n}^{t+1}}(s,a^{\prime}) \right) &\le \max_{a^{\prime}} \tau^{-1}_{t+1} f_{\theta_{n}^{t+1}}(s,a^{\prime}) + \log \left\vert \mathcal{A} \right\vert. \label{eq:log-sum}
\end{alignat}
By the log-sum-exp trick, we can obtain
\begin{alignat}{1}
- \log \sum_{a^{\prime}} \exp \left( \tau^{-1}_{t+1} f_{\theta^{t+1}}(s,a^{\prime}) \right) &\le - \frac{1}{\left\vert \mathcal{A} \right\vert} \sum_{a^{\prime}} \tau^{-1}_{t+1} f_{\theta^{t+1}}(s,a^{\prime}) - \log \left\vert \mathcal{A} \right\vert. \label{eq:log-sum-exp}
\end{alignat}
By substituting (\ref{eq:log-sum}) and (\ref{eq:log-sum-exp}) into (\ref{eq:proof:lemma:omega0}) and denoting $a_{\max} = \arg\max_{a} \tau^{-1}_{t+1} f_{\theta_{n}^{t+1}}(s,a)$ given state $s$, we have
\begin{alignat}{1}
\Omega^{t+1} &= \sum_{s} \sum_{n} q_{n} \rho_{\pi^{\ast},n}(s) \left< \log \left( \pi^{\theta^{t+1}}(\cdot \vert s) / \pi^{\theta^{t+1}_{n}}(\cdot \vert s) \right), \pi^{\ast} \right> \nonumber \\
&\le \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \tau^{-1}_{t+1} f_{\theta^{t+1}}(s,a) - \tau^{-1}_{t+1} f_{\theta_{n}^{t+1}}(s,a) + \tau^{-1}_{t+1} f_{\theta_{n}^{t+1}}(s,a_{\max}) - \frac{\sum_{a^{\prime}} \tau^{-1}_{t+1} f_{\theta^{t+1}}(s,a^{\prime})}{\left\vert \mathcal{A} \right\vert} \right] \\
&= \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \tau^{-1}_{t+1} f_{\theta^{t+1}}(s,a) - \tau^{-1}_{t+1} f_{\theta_{n}^{t+1}}(s,a) + \tau^{-1}_{t+1} f_{\theta_{n}^{t+1}}(s,a_{\max}) - \tau^{-1}_{t+1} f_{\theta_{n}^{t+1}}(s,a) \right. \nonumber \\
& \left. \quad + \tau^{-1}_{t+1} f_{\theta_{n}^{t+1}}(s,a) - \tau^{-1}_{t+1} f_{\theta^{t+1}}(s,a) - \frac{\sum_{a^{\prime}} \left( \tau^{-1}_{t+1} f_{\theta^{t+1}}(s,a^{\prime}) - \tau^{-1}_{t+1} f_{\theta^{t+1}}(s,a) \right)} {\left\vert \mathcal{A} \right\vert} \right].
\end{alignat}
By the triangle inequality, we can obtain
\begin{alignat}{1}
\Omega^{t+1} &\le \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \tau^{-1}_{t+1} f_{\theta^{t+1}}(s,a) - \tau^{-1}_{t+1} f_{\theta_{n}^{t+1}}(s,a) + \tau^{-1}_{t+1} f_{\theta_{n}^{t+1}}(s,a_{\max}) - \tau^{-1}_{t+1} f_{\theta_{n}^{t+1}}(s,a) \right. \right. \nonumber \\
& \left. \left. \quad + \tau^{-1}_{t+1} f_{\theta_{n}^{t+1}}(s,a) - \tau^{-1}_{t+1} f_{\theta^{t+1}}(s,a) - \frac{\sum_{a^{\prime}} \left( \tau^{-1}_{t+1} f_{\theta^{t+1}}(s,a^{\prime}) - \tau^{-1}_{t+1} f_{\theta^{t+1}}(s,a) \right)} {\left\vert \mathcal{A} \right\vert} 
\right\vert \right] \\
&\le \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \tau^{-1}_{t+1} f_{\theta^{t+1}}(s,a) - \tau^{-1}_{t+1} f_{\theta_{n}^{t+1}}(s,a) \right\vert + \left\vert \tau^{-1}_{t+1} f_{\theta_{n}^{t+1}}(s,a_{\max}) - \tau^{-1}_{t+1} f_{\theta_{n}^{t+1}}(s,a) \right\vert \right. \nonumber \\
& \left. \quad + \left\vert \tau^{-1}_{t+1} f_{\theta_{n}^{t+1}}(s,a) - \tau^{-1}_{t+1} f_{\theta^{t+1}}(s,a) \right\vert + \left\vert \frac{\sum_{a^{\prime}} \left( \tau^{-1}_{t+1} f_{\theta^{t+1}}(s,a^{\prime}) - \tau^{-1}_{t+1} f_{\theta^{t+1}}(s,a) \right)} {\left\vert \mathcal{A} \right\vert} 
\right\vert \right].
\end{alignat}
By Lemma \ref{lemma:changing_action_error} and Lemma \ref{lemma:aggregation_error}, we can obtain
\begin{alignat}{1}
\Omega^{t+1} &\le 4 \mathbb{E}_{n \thicksim C} \left[ \tau_{t+1}^{-1} \epsilon^{t+1}_{n} \xi^{t+1}_{n} \right] + 2 \beta_{t}^{-1} \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \sum_{i} q_{i} \left\vert Q^{w^{t}_{n}}(s,a) - Q^{w^{t}_{i}}(s,a) \right\vert \right] \nonumber \\
& \quad + 4 \tau_{t+1}^{-1} R_{\theta} + \mathcal{O} \left( \tau_{t+1}^{-1} R_{\theta}^{3/2} m^{-1/4} \right)
\end{alignat}
for the baseline and
\begin{alignat}{1}
\Omega^{t+1} &\le 4 \mathbb{E}_{n \thicksim C} \left[ \tau_{t+1}^{-1} \epsilon^{t+1}_{n} \xi^{t+1}_{n} \right] +  + 4 \tau_{t+1}^{-1} R_{\theta} + \mathcal{O} \left( \tau_{t+1}^{-1} R_{\theta}^{3/2} m^{-1/4} \right)
\end{alignat}
for FedRAC.

For Gaussian policy, we have
\begin{alignat}{1}
\Omega^{t+1} &= \sum_{s} \sum_{n} q_{n} \rho_{\pi^{\ast},n}(s) \left< \log \left( \pi^{\theta^{t+1}}(\cdot \vert s) / \pi^{\theta^{t+1}_{n}}(\cdot \vert s) \right), \pi^{\ast} \right> \\
&= \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \log \pi^{\theta_{n}^{t+1}} - \log \pi^{\theta^{t+1}} \right] \\
&= \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ - \frac{\left( a - f_{\theta^{t+1}_{n}}(s,a) \right)^2}{2 \sigma_{t+1}^{2}} - \log \sqrt{2 \pi} \sigma_{t+1} + \frac{\left( a - f_{\theta^{t+1}}(s,a) \right)^2}{2 \sigma_{t+1}^{2}} + \log \sqrt{2 \pi} \sigma_{t+1} \right] \\
&= \frac{1}{2 \sigma_{t+1}^{2}} \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left( a - f_{\theta^{t+1}}(s,a) \right)^2 - \left( a - f_{\theta^{t+1}_{n}}(s,a) \right)^2 \right].
\end{alignat}
By utilizing Taylor expansion, we can obtain
\begin{alignat}{1}
\Omega^{t+1} &= \frac{1}{2 \sigma_{t+1}^{2}} \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left( a - f_{\theta^{0}}(s,a) \right)^2 + 2 \left( f_{\theta^{0}}(s,a) - a \right) \left( f_{\theta^{t+1}}(s,a) - f_{\theta^{0}}(s,a) \right) \right. \\
& \quad + 2 \left( f_{\theta^{t+1}}(s,a) - f_{\theta^{0}}(s,a) \right)^{2} - \left( a - f_{\theta^{0}}(s,a) \right)^2 - 2 \left( f_{\theta^{0}}(s,a) - a \right) \left( f_{\theta^{t+1}_{n}}(s,a) - f_{\theta^{0}}(s,a) \right) \\
& \quad \left. - 2 \left( f_{\theta^{t+1}_{n}}(s,a) - f_{\theta^{0}}(s,a) \right)^2 \right] \\
&= \frac{1}{2 \sigma_{t+1}^{2}} \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ 2 \left( f_{\theta^{0}}(s,a) - a \right) \left( f_{\theta^{t+1}}(s,a) - f_{\theta^{t+1}_{n}}(s,a) \right) \right. \\
& \quad \left. + 2 \left( f_{\theta^{t+1}}(s,a) - f_{\theta^{0}}(s,a) \right)^{2} - 2 \left( f_{\theta^{t+1}_{n}}(s,a) - f_{\theta^{0}}(s,a) \right)^2 \right] \\
&\le \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \frac{f_{\theta^{0}}(s,a) - a}{\sigma_{t+1}^{2}} \left( f_{\theta^{t+1}}(s,a) - f_{\theta^{t+1}_{n}}(s,a) \right) \right] + \frac{R_{\theta}^{2}}{\sigma_{t+1}^{2}} \\
&\le \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \left\vert \upsilon_{t+1}^{-1}(s,a) f_{\theta^{t+1}}(s,a) - \upsilon_{t+1}^{-1}(s,a) f_{\theta^{t+1}_{n}}(s,a) \right\vert \right] + \frac{R_{\theta}^{2}}{\sigma_{t+1}^{2}}.
\end{alignat}
By Lemma \ref{lemma:aggregation_error}, we can obtain
\begin{alignat}{1}
\Omega^{t+1} &\le 2 \mathbb{E}_{n \thicksim C} \left[ \sup \left\vert \upsilon_{t+1}^{-1}(s,a) \right\vert \tilde{\epsilon}_{n}^{t+1} \xi^{t+1}_{n} \right] + \beta_{t}^{-1} \mathbb{E}_{n \thicksim C, s \thicksim \rho_{\pi^{\ast},n}, a \thicksim \pi^{\ast}} \left[ \sum_{i} q_{i} \left\vert Q^{w^{t}_{n}}(s,a) - Q^{w^{t}_{i}}(s,a) \right\vert \right] \nonumber \\
& + \mathcal{O} \left( \sup \left\vert \upsilon_{t+1}^{-1}(s,a) \right\vert R_{\theta}^{3/2} m^{-1/4} \right) + \frac{R_{\theta}^{2}}{\sigma_{t+1}^{2}}
\end{alignat}
for the baseline and
\begin{alignat}{1}
\Omega^{t+1} &\le 2 \mathbb{E}_{n \thicksim C} \left[ \sup \left\vert \upsilon_{t+1}^{-1}(s,a) \right\vert \tilde{\epsilon}_{n}^{t+1} \xi^{t+1}_{n} \right] + \mathcal{O} \left( \sup \left\vert \upsilon_{t+1}^{-1}(s,a) \right\vert R_{\theta}^{3/2} m^{-1/4} \right) + \frac{R_{\theta}^{2}}{\sigma_{t+1}^{2}}
\end{alignat}
for FedRAC.
\end{proof}

We study the Proximal Policy Optimization (PPO) algorithm within the Federated Reinforcement Learning (FRL) framework. As an Actor-Critic style algorithm, PPO's conventional update rule (Critic first, Actor follows) does not correspond with the FRL objective, which encompasses heterogeneous local objectives. The heterogeneity leads to divergent gradient directions among clients, impeding convergence to the globally optimal policy. Compared with federated supervised learning where gradients are locally estimated from private data, the Actor-Critic structure of PPO enables us to share information about gradients or objectives via the action-value function without violating data privacy. In light of this, we propose FedRAC which reverses the update order (Actor first, Critic follows) to synchronize the action-value function better. The theoretical analysis reveals that the proposed method demonstrates reduced sensitivity to heterogeneity. Moreover, its convergence bound is primarily influenced by the aggregation error, which depends on the linearity of the underlying function approximation. Empirical results indicate that the proposed algorithm converges more swiftly in three toy environments and within a highly heterogeneous network utilizing the SUMO traffic simulator.

\begin{alignat}{1}
\upsilon_{t}(s,a) &= \frac{\sigma_{t}^{2}}{a - f_{\theta^{0}}(s,a)}, \\
\phi^{t+1}_{n} &= \mathbb{E}_{s \thicksim \rho_{\pi^{\theta^{t}},n}, a \thicksim \pi^{\theta^{t}}} \left[ \left( \log \frac{\sigma_{t}}{\sigma_{t+1}} \right. \right. \nonumber \\
& \quad \left. \left. + \frac{1}{2}\left( \frac{1}{\sigma_{t+1}^{2}} - \frac{1}{\sigma_{t}^{2}} \right)\left( f_{\theta^{0}}^{2} - a^{2} \right) \right)^{2} \right], \\
\tilde{\epsilon}_{n}^{t+1} &= \sqrt{\left( \frac{\tau_{t+1}^{-1} \epsilon_{n}^{t+1}}{3} \right)^{2} - \phi^{t+1}_{n} - \frac{R_{\theta}^{4}}{4 \sigma_{t+1}^{4}}}, \\
\hat{\epsilon}_{n}^{t+1} &= \frac{(\dot{\epsilon}_{n}^{t+1})^{2} - 8 R_{w}^{2}}{\mathbb{E}_{i} \left[ \left\vert \frac{\rho_{\pi^{\ast},n}(s)}{\rho_{\pi^{\ast},i}(s)} \right\vert^{2} \right]^{1/2} 4 \mathbb{E}_{i} \left[ \left\vert \frac{\rho_{\pi^{\ast},i}(s)}{Z_{\pi^{\ast}}(s)} \right\vert^{8} \right]^{1/4} } \nonumber \\
& \quad - \frac{\mathbb{E}_{i} \left[ \left\vert Q^{\pi^{\theta^{t}}}_{i} \right\vert^{4} \left\vert 1 -\frac{\rho_{\pi^{\ast},i}(s)}{Z_{\pi^{\ast}}(s)} \right\vert^{4} \right]^{1/2} }{\mathbb{E}_{i} \left[ \left\vert \frac{\rho_{\pi^{\ast},i}(s)}{Z_{\pi^{\ast}}(s)} \right\vert^{8} \right]^{1/4} }.
% \frac{(\epsilon_{n}^{t+1})^{2} - \phi^{t+1}_{n}}{\mathbb{E}_{s \thicksim \rho_{\pi^{\theta^{t}},n}, a \thicksim \pi^{\theta^{t}}} \left[ (\upsilon_{t+1}(s,a))^{-4} \right]^{1/2}}.
\end{alignat}

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
